The quest for scaling BFT Consensus through Tree-Based Vote Aggregation

With the growing commercial interest in blockchain, permissioned implementations have received increasing attention. Unfortunately, existing BFT consensus protocols that are the backbone of permissioned blockchains, either scale poorly or offer limited throughput. Most of these algorithms require at least one process to receive and validate the votes from all other processes and then broadcast the result, which is inherently non-scalable. Some algorithms avoid this bottleneck by using aggregation trees to collect and validate votes. However, to the best of our knowledge, such algorithms offer limited throughput and degrade quickly in the presence of faults. In this paper we propose \thesystem, the first BFT communication abstraction that organizes participants in a tree to perform scalable vote aggregation and that, in faulty runs, is able to terminate the protocol within an optimal number of reconfigurations ($f+1$). We define precisely which aggregation trees allow for optimal reconfiguration and show that, unlike previous protocols, when using these configurations, \thesystem scales to large number of processes and outperforms HotStuff's throughput by up to 38x.

==> abstractions.tex <==
\subsection{Abstractions}
\label{sec:abstractions}

We now introduce a set of abstractions to reason about the use of trees in the context of consensus protocols. Namely, we define and introduce the properties of robust graphs, the communication primitives and the cryptographic abstractions.
In the next section, we show how these abstractions are used to implement \thesystem.

Processes are organized in overlay networks that are used to disseminate messages. Note that we assume that the underlying physical network is a clique, allowing every process to communicate directly with each other if needed. 
%We define and use multiple overlay networks: each overlay network defines a given configuration (or view). 
%As all leader-based consensus protocols, \thesystem requires a view change sub-protocol, used for re-configuring the overlay network used for consensus. As we will discuss later, the view-change protocol uses the underlying clique and not one of the overlay networks.

The overlay network used to support the communication among participants in \thesystem can be modelled as a graph, where each process maps to one and only one vertex in the graph. In  \thesystem, we only use graphs that are undirected and acyclic. 
Furthermore, from all the possible graphs, consensus is only guaranteed to terminate if participants eventually use a configuration where the overlay network corresponds to a \textit{robust graph}.

\begin{definition}
\textbf{Robust Graph:} An edge is said to be \textit{safe} if the corresponding vertices are both correct processes. A graph is robust iff for every pair of correct process $p_i$ and $p_j$, there is a path between $p_i$ and $p_j$ composed exclusively of safe edges. \label{def:robust}
\end{definition}

\mm{note to self: introduce main alg. here assuming a robust graph}


\subsubsection{Recurringly Robust Evolving Graph}

Even if we start from a robust graph, due to faults, \thesystem may be required to perform one or more reconfigurations of the graph (or view changes). 
Every reconfiguration defines a new overlay network that will be used by the processes to communicate. 
We can model the sequence of overlay networks used by \thesystem as an evolving graph, i.e., a sequence of static graphs. To ensure that eventually a robust graph is used, the evolving graph must hold the following property:

\begin{definition} 
\textbf{Recurringly Robust Evolving Graph:} An evolving graph $\mathcal{G}$ is denoted to be \textit{recurringly robust} iff robust static graphs appear infinitely often in its sequence. \label{def:recurringlyrobust}
\end{definition}

\subsubsection{$t$-Bounded Conformity}

Note that even though a recurringly robust evolving graph is sufficient to ensure that a robust graph will be eventually used by processes to communicate, it is not very interesting in practice because the number of reconfigurations that are necessary before a robust graph is found are potentially unbound. Ideally, we would like the system to use a robust graph after at most $t$ reconfigurations. We call this property of an evolving graph \textit{$t$-bounded conformity}. 

\begin{definition}
\textbf{$t$-Bounded Conformity}: a recurringly robust evolving graph $\mathcal{G}$ exhibits \textit{$t$-bounded conformity} if a robust static graph appears in $\mathcal{G}$ at least once every $t$ consecutive static graphs.\label{def:boundedconformity}
\end{definition}

Note that, in the worst case, any leader-based protocol may require at least $f+1$ reconfigurations, because a faulty leader can always prevent consensus from being reached in which case it needs to be replaced. Interestingly, for general topologies it may be hard, or even impossible to achieve $t$-bounded conformity. Consider, for instance, an evolving graph where all static graphs are binary trees. The number of possible binary trees is factorial with the number of processes and, from all these trees, only a small fraction is robust - i.e. those where faulty processes are not interior nodes. A naive evolving graph that is constructed by a simple permutation among all possible configurations of the tree could require therefore a factorial number of reconfigurations to find a robust graph. 

Ideally, we want to have a bound number of reconfigurations such that they grow linearly either with the size of the system $N$ or the number of faults $f$.
This leads us to the notion of \emph{Linear Conformity} and \emph{Optimal Conformity}, respectively, as defined below.
%Therefore, in a system where $f$ processes may be faulty, we ideally want to build an evolving graph that observes 
%\emph{Optimal Conformity}.

\begin{definition}
\textbf{Linear Conformity}: a recurringly robust evolving graph $\mathcal{G}$ has Linear conformity iff, $\mathcal{G}$ observes $t$-bounded conformity where $t=\mathcal{O}(N)$.
\label{def:optimalconformity}
\end{definition}

\begin{definition}
\textbf{Optimal Conformity}: a recurringly robust evolving graph $\mathcal{G}$ has Optimal conformity iff $\mathcal{G}$ observes $t$-bounded conformity where $t=f+1$ with $f=\floor{\frac{N-1}{3}}$.
\label{def:optimalconformity}
\end{definition}

\subsubsection{Communicating on the Graph}
Processes use the overlay network to communicate. \thesystem assumes the availability of perfect point-to-point channels that are implemented on each edge of the overlay network. and used by processes to communicate with each neighbor. Each directed edge is used at most once, to send and deliver a single value. Perfect point-to-point channels expose a \textsc{send} primitive used to send a message, and a \textsc{deliver} primitive used to receive a message, and exhibit the following properties.

\begin{itemize}
    \item \emph{Validity:} If a process $p_j$ delivers a value $v$ on a channel over an edge $e_{ij}$, $v$ was sent by $p_i$.
    \item \emph{Termination:} If both $p_i$ and $p_j$ are correct, if $p_i$ invokes \textsc{send} then eventually $p_j$ delivers $v$.
\end{itemize}

%When using the overlay to aggregate information, nodes wait for their children to propagate data upstream. Conversely, when the overlay is used to dissiminate information, nodes wait for their parents to propagate downstream. For liveness, the aggregation/dissemination process must proceed even in the occurrence of faults. 
Note that, when using perfect channels, a message is only guaranteed to be eventually delivered if both the sender and the recipient are correct. If the sender is faulty, no message may ever be delivered. To avoid blocking, a process should be able to make progress if a message takes too long to be received.

This behaviour is captured by an abstraction we call \textit{impatient channels}. Impatient channels offer a blocking \textsc{receive} primitive that always returns a value: either the value sent by the sender, or a special value  $\bot$ if the sender is faulty or the system is unstable. After the Global Stabilization Time (GST)\cite{partial}, if the sender and the receiver are correct, the receiver always receives the value sent. Impatient channels have the following properties:

\begin{itemize}
    \item \emph{Validity:}  If a process $p_j$ receives a value $v$,  $v$ was sent by a process $p_i$ or $v=\bot$.
    \item \emph{Termination:}  If a correct process $p_j$ invokes \textsc{receive}, it eventually returns some value.
    \item \emph{Conditional Accuracy:} Let $p_i$ and $p_j$ be correct sender and receiver processes, respectively. After GST, $p_j$ always return the value $v$ sent by $p_i$.
\end{itemize}

Algorithm~\ref{algo:impchannels-receive} shows how impatient channels can be implemented on top of perfect channels using the known bound $\Delta$ on the worst-case network latency.

\setlength{\textfloatsep}{0pt}
\begin{algorithm}[t]
\scriptsize
\centering
\caption{Impatient Channels: implementation of \textsc{receive}}
\label{algo:impchannels-receive}
\begin{algorithmic}[1]

\State{let \textit{ic}$_{ij}$ be an impatient channel built on top of perfect channel \textit{pc}$_{ij}$}
\Function{$\textit{ic}_{ij}$\textsc{.receive}}{ }
\State{\textsc{timer.start}($\Delta$)}
\When{\textit{pc}$_{ij}$.\textsc{deliver} ($v_i$)}
    \State{\Return $v_i$}
\EndWhen
\When{\textsc{timer.timeout}()}
    \State{\Return $\bot$}
\EndWhen
\EndFunction
\end{algorithmic}
\end{algorithm}
\setlength{\textfloatsep}{5pt}

\subsubsection{Cryptographic Collections}

In each phase of the consensus protocol, it is necessary to collect a Byzantine quorum of votes. The collection, and validation, of these votes can be an impairment for scalability. \thesystem mitigates these costs by using the overlay network to aggregate votes as they are forwarded to the leader. We model the process of aggregation of votes using an abstraction that we named a \textit{cryptographic collection}, which models a secure multi-set of tuples $(p_i, v_i)$. A process $p_i$ can create a new collection $c$ with a value $v_i$ by calling $c$=\textsc{new}($(p_i, v_i)$). Processes can also merge two collections using a \textsc{combine} primitive,  $c_{12}$ = \textsc{combine}$(c_1, c_2)$, also denoted by $c_{12} = c_1 \oplus c_2$. Finally, a process can check if a collection $c$ includes at least a given threshold of $t$ distinct tuples with the same value $v$, by calling \textsc{has}$(c, v, t)$. Additionally, it is possible to check the total amount of input tuples that were contributed to $c$ by checking its cardinality $\vert c \vert$. Cryptographic collections have the following properties:

\begin{itemize}
    \item \emph{Commutativity:}   $c_1 \oplus c_2 = c_2 \oplus c_1$.
    \item \emph{Associativity:}   $c_1 \oplus (c_2 \oplus c_3)  = (c_1 \oplus c_2) \oplus c_3$.
    \item \emph{Idempotency:} $c_1 \oplus c_1 = c_1$.
    \item \emph{Integrity:} Let $c= c_1 \oplus \ldots c_i \ldots c_n$. If \textsc{has} ($c, v, t$) then at least $t$ distinct processes $p_i$ have executed $c_i$=\textsc{new}($(p_i, v)$).
\end{itemize}

Note that different cryptographic techniques can be used to implement these collections. In \thesystem, we leverage the BLS non-interactive cryptographic aggregation scheme that allows each inner node to aggregate the votes from its children into a single aggregated vote~\cite{bls}. The complexity of verifying an aggregated vote is $\mathcal{O}(1)$, thus the burden imposed on each inner node (including the root) is $\mathcal{O}(c)$, where $c$ is the fanout of the tree.  Note that classical asymmetric signatures require $\mathcal{O}(N)$ verifications at every process and threshold signature schemes require $\mathcal{O}(N)$ at the root and $\mathcal{O}(1)$ at all the other processes~\cite{bls}.

==> hotstuff.tex <==
%todo work a bit on this
%todo, make an algo that implements "broadcast" and "send to leader" and uses the tree build alg and the cryptographic primitives.


\setlength{\textfloatsep}{0pt}
\begin{algorithm}[h!]
\scriptsize
\centering
\caption{HotStuff Consensus Algorithm}
\label{algo:consensusalgo}
\begin{algorithmic}[1]
\State{blockchain $\gets b_0$} \Comment{Local blockchain, initially with the genesis block $b_0$}
\State{view $\gets \ldots$} \Comment{Local view}
\State{id $\gets \ldots$} \Comment{The id of this process}
\State{prepareQC $\gets \varnothing$} \Comment{Prepare quorum commitment}
\State{lockQC $\gets \varnothing$} \Comment{Lock quorum commitment}
\State{highQC $\gets \varnothing$}

\Upon{\textsc{init}} {} \label{algo2:line:init}
\If{$view.leader(id)$}
\State{blockchain.createBlock()}
\State{\textbf{broadcast} (\textsc{prepare}, blockchain.getTopBlock())}
\EndIf
\EndUpon \label{algo2:line:init-end}

\Upon{\textsc{receive} $block^{prepare}_i$} { } \Comment{On Receiving block proposal} \label{algo2:line:receiveblock}
\If{$b_i$.isValid() $\land b_i$.parent = blockchain.getTopBlock()}
\State{blockchain.append($block^{prepare}_i$)}
\State{\textbf{send} (\textsc{prepare}, sign($b_i$)) \textbf{to leader}}
\EndIf
\EndUpon \label{algo2:line:receiveblock-end}

\Upon{\textsc{receive} $vote^{prepare}_i$} { } \Comment{On receiving prepare vote} \label{algo2:line:receivepreparevote}
\If{verify($vote^{prepare}_i$)}
\State{blockchain.getTopBlock().addSignature(\textsc{prepare}, $vote^{prepare}_i$)}
\If{$\vert$blockchain.getTopBlock().getQC(\textsc{prepare})$\vert \geq 2f+1$ }
\State{prepareQC $\gets$ blockchain.getTopBlock().getQC(\textsc{prepare})}
\State{\textbf{broadcast} (\textsc{precommit}, prepareQC)}
\EndIf
\EndIf
\EndUpon \label{algo2:line:receivepreparevote-end}

\Upon{\textsc{receive} $qc^{precommit}_i$} { } \Comment{On Receiving pre-commit QC} \label{algo2:line:receiveprecommit}
\If{verify($qc^{precommit}_i$)}
\State{prepareQC $\gets qc^{precommit}_i$}
\State{\textbf{send} (\textsc{precommit}, sign($qc^{precommit}_i$)) \textbf{to leader}}
\EndIf
\EndUpon \label{algo2:line:receiveprecommit-end}

\Upon{\textsc{receive} $vote^{precommit}_i$} { } \Comment{On receiving pre-commit vote} \label{algo2:line:receiveprecommitvote}
\If{verify($vote^{precommit}_i$)}
\State{blockchain.getTopBlock().addSignature(\textsc{precommit}, $vote^{precommit}_i$)}
\If{$\vert$blockchain.getTopBlock().getQC(\textsc{precommit})$\vert \geq 2f+1$ }
\State{lockedQC $\gets$ blockchain.getTopBlock().getQC(\textsc{precommit})}
\State{\textbf{broadcast} (\textsc{commit}, lockedQC)}
\EndIf
\EndIf
\EndUpon \label{algo2:line:receiveprecommitvote-end}

\Upon{\textsc{receive} $qc^{commit}_i$} { } \Comment{On Receiving commit QC} \label{algo2:line:receivecommit}
\If{verify($qc^{commit}_i$)}
\State{lockedQC $\gets qc^{commit}_i$}
\State{\textbf{send} (\textsc{commit}, sign($qc^{commit}_i$)) \textbf{to leader}}
\EndIf
\EndUpon \label{algo2:line:receivecommit-end}

\Upon{\textsc{receive} $vote^{commit}_i$} { } \Comment{On receiving commit vote} \label{algo2:line:receivecommitvote}
\If{verify($vote^{commit}_i$)}
\State{blockchain.getTopBlock().addSignature(\textsc{commit}, $vote^{commit}_i$)}
\If{$\vert$blockchain.getTopBlock().getQC(\textsc{commit})$\vert \geq 2f+1$ }
\State{blockchain.getTopBlock().finalize()}
\State{\textbf{broadcast} (\textsc{decide}, blockchain.getTopBlock().getQC(\textsc{commit}))}
\EndIf
\EndIf
\EndUpon \label{algo2:line:receivecommitvote-end}

\Upon{\textsc{receive} $qc^{decide}_i$} { } \Comment{On Receiving decide QC} \label{algo2:line:receivedecide}
\If{verify($qc^{decide}_i$)}
\State{blockchain.getTopBlock().finalize()}
\State{\textbf{send} (\textsc{newview}, sign($lockedQC$)) \textbf{to leader}}
\EndIf
\EndUpon \label{algo2:line:receivedecide-end}

\Upon{\textsc{receive} $vote^{new-view}_i$} { } \Comment{On receiving vote at the leader} \label{algo2:line:receivenewviewvote}
\If{verify($vote^{new-view}_i$)}
\State{highQC.addSignature($vote^{new-view}_i$)}
\If{$\vert$highQC$\vert \geq 2f+1$ }
\State{blockchain.createBlock(\textsc{max}(highQC)))}
\State{\textbf{broadcast} (\textsc{prepare}, blockchain.getTopBlock())}
\EndIf
\EndIf
\EndUpon \label{algo2:line:receivenewviewvote-end}

\end{algorithmic}
\end{algorithm}

==> older-versions/abstract-202011061420.tex <==

\begin{abstract}
Permissioned blockchains have several advantages over permissionless blockchains, in particular, they are able to ensure finality, i.e., to prevent forks that may cause committed transactions to be undone. This has raised an increasing interest in finding techniques that can make byzantine fault-tolerant consensus scale to large numbers of participants, a setting that is common in existing blockchains. Classical Byzantine consensus protocols, such as PBFT, organize participants in a clique and have quadratic message complexity. More recent algorithms, such as HotStuff, organize participants in a star topology, which allows to reduce the message complexity but fails to reduce the load on the coordinator, that is still required to receive and validate votes from all other processes. These algorithms are, therefore, inherently non-scalable. The use of aggregation trees to collect votes has the potential for deriving scalable algorithms but also makes the consensus less robust: a faulty interior node may prevent aggregation to terminate. To the best of our knowledge, previous algorithms that explore the use of trees to aggregate votes always fall back in faulty-runs to non-scalable topologies, such as a clique or a star. In this paper we propose \thesystem, the first BFT consensus protocol that organizes participants in a tree to perform scalable vote aggregation while still converging to a (tree-based) robust configuration in optimal number of steps $\mathcal{O}(t)$. We define precisely which aggregation trees allow for optimal reconfiguration and show that, unlike previous protocols, when using these configurations, \thesystem can offer large throughput in settings up to XXX participants.
\end{abstract}


\begin{IEEEkeywords}
Byzantine Fault Tolerance, Consensus, Blockchain, Distributed Ledger, Communication Graph
\end{IEEEkeywords}



%\begin{abstract}

%[Ray's version] In recent years there has been a significant amount of research regarding the use of consensus to implement distributed ledgers. Classical Byzantine consensus protocols, such as PBFT, assume that processes are organized in a clique topology, and use an all-to-all communication pattern resulting in a quadratic number of messages. This is often unfeasible in the context of distributed ledgers, where the number of participants may be large. Because of this, several algorithms that exploit different communication topologies have been proposed, aiming to reduce the message complexity and/or to offer better load balancing properties. In this context, the use of a star topology that results in a linear communication complexity has shown to scale very well.
%However, requiring the central process to receive, verify and aggregate the signatures of all participants quickly leads to a performance bottleneck. Due to this, alternative topologies, such as trees, have been proposed in the literature that balance the load over a set of processes.

%However, existing approaches that leverage tree structures fall-back to a star or clique relatively quickly in the presence of failures and it is unclear how these protocols return to the tree structure eventually. Not only that, but to the best of our knowledge, none of the existing works compare their approaches to high throughput solutions in the literature which makes it difficult to reason about the actual scalability and viability of these approaches.

%Therefore, in this paper, we present \thesystem a high throughput byzantine fault tolerant consensus algorithm that leverages trees to achieve high scalability. We compare \thesystem to \textit{HotStuff} a state of the art consensus algorithm that leverages a star topology.  %TODO: More exact numbers%
%Our experiments show that \thesystem outperforms \textit{HotStuff} in several setups and scales significantly better to large groups of processes.

%As a result of this, traditional byzantine fault tolerant consensus can be scaled more easily to large groups of processes making it more viable to be used in large scale use cases.
%\end{abstract}

==> older-versions/abstract-202012211500.tex <==
%\begin{abstract}
%Permissioned blockchains have several advantages over permissionless blockchains, in particular, they are able to ensure finality, i.e., to prevent forks that may cause committed transactions to be undone. This has raised an increasing interest in finding techniques that can also make permissioned byzantine fault-tolerant consensus scale to large numbers of participants, as is common in most existing permissionless blockchains. Classical Byzantine consensus protocols, such as PBFT, organize participants in a clique with a quadratic message complexity. More recent algorithms, such as HotStuff, organize participants in a star topology reducing the message complexity but failing to reduce the load on the coordinator, that is still required to receive and validate votes from all other processes. These algorithms are, therefore, inherently non-scalable. The use of aggregation trees to collect votes has the potential for deriving scalable algorithms but is also less robust: a faulty internal node in a tree may impede the aggregation. To the best of our knowledge, previous algorithms that leverage trees to aggregate votes always fall back to a clique or a star in faulty-runs. Additionally, these algorithms, due to the additional communication steps, reduce the throughput of the overall protocol. In this paper we propose \thesystem, the first BFT communication abstraction that organizes participants in a tree to perform scalable vote aggregation and that, in faulty runs, is able to reconfigure the tree in optimal steps ($f+1$). We define precisely which aggregation trees allow for optimal reconfiguration and show that, unlike previous protocols, when using these configurations, \thesystem scales to large number of processes and offers, depending on the deployment scenario, up to 17 times higher throughput than HotStuff.
%\end{abstract}


\begin{abstract}
With the growing interest of big companies in blockchain use-cases, permissioned blockchains have received increasing attention. However, existing byzantine fault tolerant consensus protocols, that are the backbone of permissioned blockchains, either scale badly to large system sizes or offer limited throughput.
Most of these algorithms require one or more processes to receive and validate the votes from all other processes and then broadcast the result, which is inherently non-scalable. Other algorithms use aggregation trees to collect and validate votes to balance the load. However, to the best of our knowledge, these algorithms always fall back to a clique or a star in faulty-runs. Additionally, due to the additional communication steps, with increasing latency, they are unable to provide throughput comparable to the broadcast based systems. 
In this paper we propose \thesystem, the first BFT communication abstraction that organizes participants in a tree to perform scalable vote aggregation and that, in faulty runs, is able to reconfigure the tree in optimal steps ($f+1$). We define precisely which aggregation trees allow for optimal reconfiguration and show that, unlike previous protocols, when using these configurations, \thesystem scales to large number of processes and offers, depending on the deployment scenario, up to 17 times higher throughput than HotStuff even with increased latency and communication steps.


\end{abstract}

\begin{IEEEkeywords}
Byzantine Fault Tolerance, Consensus, Blockchain, Distributed Ledger, Communication Graph
\end{IEEEkeywords}


==> older-versions/evaluation-202012291545.tex <==
\section{Evaluation}
\label{sec:evaluation}

While in the previous sections, we've always assumed perfect balanced \textit{m-ary} trees, we know that in practise it is very unlikely to have the exact number of processes for such a deployment.

In practise a maximum fanout depending on the bandwidth and fault tolerance requirements has to be selected. Based on this, nodes are equally distributed down the tree to approximate a balanced tree.
While this might result in suboptimal trees where internal nodes at the lowest level might have only 1-2 child processes, due to the pipelining scheme the additional latency cost is easily compensated.

In our experiments, we, therefore, have chosen practical deployment sizes of $100, 200$ and $400$ processes and a fixed depth of $h=3$. The fanout at the root was adjusted to find the maximum throughput and the leave processes were distributed equally over the internal nodes. 
This resulted in a varied fanout depending on the system size and the scenario (fanout of 20 for 400 processes, 15-20 for 200 processes and 10 for 100 processes).

Additionally, we've varied the number of concurrent blocks through pipelining until the system was saturated.

In this section we evaluate the performance of our approach and prototype and put it in relation to HotStuff. More specifically we will:

\begin{enumerate}
    \item Assess the performance of different cryptographic operations to establish a baseline;
    \item Evaluate how the prototype compares to HotStuff;
    \item Evaluate the impact of the pipelining.
\end{enumerate}

Experiments presented in this paper were carried out on the Grid'5000 testbed, supported by a scientific interest group hosted by Inria and including CNRS, RENATER and several Universities as well as other organizations~\cite{grid5000}.
Each of the physical machines runs on two Intel Xeon E5-2620 v4 8-core CPUs with 64 GiB RAM. We've reserved up to 12 physical machines and, thus to scale the experimental setting, co-located always around 40 consensus processes. The center node of the star and the root node of the tree ran on separate physical machines individually. In order to avoid short communication paths within a physical machine, nodes ran on separate machines than their respective children and parents.

In order to simulate bandwidth and latency restrictions we used the native \textit{netem} tool on linux. We've restricted the latency at each individual machine and the bandwidth at the root/center process. We've considered a total of three different latency/bandwidth scenarios we've picked from the literature and actual use-cases. The first scenario is the use-case of a globally distributed blockchain similarly as proposed in \cite{motor, algorand, byzcoin} with $200ms$ roundtrip latency and $25mbit/s$ bandwidth. The remaining use-cases were picked from industry use-case scenarios reported in \cite{blockchain50}.
Based on this, the next scenarios assume a reduced geographical distribution, for example for local supply-chain management, exchange of medical data, or digital currency (E-Euro, or E-Dollar). First, we got an US or EU wide scenario with a max of $100ms$ latency and $100mbit/s$ bandwidth and finally we got one country-wide (Germany, France, GB, etc) scenarios with $20ms$ roundtrip latency and $100mbit/s$ bandwidth.

Due to those restrictions, the results presented below show a significantly lower throughput than the results reported in the original \textit{HotStuff} paper~\cite{yin2019hotstuff}. This is the case since in the original experiments in \cite{yin2019hotstuff} the latency between the processes was $1ms$ and the measured bandwidth usage reached peaks of over $8gb(s)$ with $128$ processes. Similarly to most scenarios in \cite{yin2019hotstuff} each block consists of $400$ operations resulting in a combined size of $100kb$.

\subsection{Practical Scalability Limits}

As identified in Section~\ref{sec:pipelining-throughput} the main scalability bottleneck of the system is the bandwidth. However, with increasing bandwidth, eventually the computing capacity also becomes a factor. Thus, in the context of the experiments we are going to execute, we have to identify the limitations of our system.

Since the most expensive operations of consensus protocols that leverage asymmetric signatures are the operations regarding these signatures (sign, verify, aggregate), we've executed this experiment to specifically assess the CPU load of the protocol. With this information in hand we can then estimate the theoretical maximum throughput.
In this context we compare the computational cost of \textit{bls signatures} with \textit{secp} and, as a baseline, with \textit{gpg}~\cite{gnupg} which is the most common cryptographic library shipped with linux.

Figure~\ref{fig:crypto} outlines the result of this experiment.
%While \textit{bls-signatures} are significantly faster in terms of signing time than \textit{gpg} it's verification time is several orders of magnitude higher.
%Meanwhile, \textit{secp} outperforms \textit{bls} both, in terms of signing and verification time, by several orders of magnitude and even has a decent advantage in terms of verification time over \textit{gpg}.
In addition to the results presented, since \textit{bls-signatures} is based on cryptographic pairings, executing multiple verifications in sequence reduces the time to approximately $3400 us$ (over 5 operations). \textit{Bls-signatures} also come with an aggregation cost for both signatures and public keys (to verify aggregates).
Similarly, due to the pairing based operations, aggregating larger numbers of elements reduces the time per element. The exact numbers for this are displayed in Figure~\ref{fig:blsagg}.

\begin{figure*}[!h]
\begin{subfigure}{0.33\textwidth}
     \centering
	\includegraphics[width=\textwidth]{figures/crypto.pdf}
	\caption{Cryptographic Operation Comparison}
  \label{fig:crypto}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
     \centering
	\includegraphics[width=\textwidth]{figures/blsagg.pdf}
	\caption{Aggregation Time Evaluation}
  \label{fig:blsagg}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
     \centering
	\includegraphics[width=\textwidth]{figures/piped.pdf}
	\caption{Different degrees of pipelining}
  \label{fig:figpiperes}
\end{subfigure}
\end{figure*}

%Assuming a system with $400$ processes, the center node of the star has to verify approximately $266$ signatures each round ($2f+1$ signatures). At $4300us$ verification time per signature this requires $1.14ms$ (not even considering aggregation time). Limiting the throughput at $400$ processes to less than one block per second.
%Using \textit{secp}, the same requires $24ms$ which is significantly less, resulting in a computational limit of approximately $42$ blocks per second.

%Considering a tree topology with a fan-out of $20$, each process has to verify and aggregate $20$ signatures resulting in approximately $86ms$ and a theoretical max of around $11$ blocks per second. With increasing system size, at around $2000$ processes, due to load balancing, the tree using \textit{bls-signatures} has a lower computational load than the star using \textit{secp}.

The above numbers are then used the in remaining evaluation section to justify and understand the experimental results. 

%\paragraph*{Bandwidth Consumption}

%While the star requires lower computational resources than the tree until approximately $2000$ processes, this is not the only potential bottleneck of the system.

%Assuming $400$ processes, at $100kbit$ per block, the center process of the star already consumes $40mbit/s$ of bandwidth per block only for the block dissemination. Additionally, using \textit{secp}, since there is no aggregation, there are $10mb$ of signatures, resulting in a total of $50mbit/s$ of bandwidth consumption. This way, even if the system could execute $166$ blocks per second, even at $1gbit/s$ of bandwidth, the system may not execute more than $20$ blocks per second.
%\thesystem on the other hand, only requires $2mbit/s$ in this scenario and would be able to execute up to $500$ blocks per second.

\subsection{Throughput Comparison}

We assess the performance of \thesystem in all three scenarios both with and without pipelining and compare it to the performance of HotStuff (with bls signatures and libsec).
Figure~\ref{fig:threescen} contains the results of this experiment. While HotStuff offers better performance in runs with low numbers of processes, with increasing number of processes this dwindles and eventually \thesystem takes over.
This is the case since with low numbers of processes the latency induced cost of the tree based protocol is larger than the bandwidth and computing bottleneck of the star. However, with increasing numbers of processes this eventually shifts.

\begin{figure}[!htb]
     \centering
	\includegraphics[width=0.75\columnwidth, height=6cm]{figures/threescen.pdf}
	\caption{Kauri vs HotStuff in 3 different Scenarios}
  \label{fig:threescen}
\end{figure}

Using pipelining (Kauri (P)), in all three experiments, as shown in Figure \ref{fig:threescen}, the throughput of \thesystem is significantly higher than the throughput of the star (independently if the star uses \textit{secp} or \textit{bls-signatures}).

As outlined before, in all scenarios, due to the large number of processes, the star bottlenecks at the bandwidth, significantly limiting its scalability. We may also observe this from the fact that the implementation of the star that uses \textit{bls-signatures} outperforms the one using \textit{secp} even though the computational cost is significantly higher. This is the case since \textit{secp} adds an additional strain on the bandwidth due to the requirement to disseminate $2f+1$ signatures each communication round.

Meanwhile, \thesystem leverages pipelining to compensate for the higher latency cost allowing it to produce a large number of blocks per second where both the computational as well as bandwidth consumption are equally distributed over the tree.

\subsection{Pipelining}

In the final experiment we aimed at asserting how the system behaves with an increasing number of additional blocks through pipelining.

We've chosen a scenario with $100ms$ roundtrip time and $100mbit/s$ bandwidth. There is a total of $200$ processes with a fan-out of $20$.
Following the theoretical model that is $2mbit$ of data per block resulting in a theoretical max of $50$ blocks per second.
Without pipelining, we produce roughly $2.5$ blocks per second resulting in a max speed up factor of $20$ in terms of bandwidth.

In terms of processing power, following the signature verification, creation and aggregation cost obtained earlier, each block requires approximately $0.1$s of processing time (sequential execution performance). Which allows for at most $4$ pipelined blocks. Due to the limited number of homogeneous physical machines we had available for the experiments we were not able to locate each internal node on a separate machine to allow higher speedup factors through increased multithreading.

Figure~\ref{fig:figpiperes} depicts the result of this experiment.
Initially, until four pipelined blocks, we are able to almost linearly increase the performance of the system with each additional block. However, as expected, with increasing numbers, as soon as we reach a certain saturation limit, the additional performance gain starts flattening off.

\subsection{Leader Replacement}

Since the system detects a non robust configuration based on timeout values it is difficult to provide a meaningful comparison, as was also pointed out in the HotStuff paper \cite{yin2019hotstuff}. This is the case, since in HotStuff and hence also in our implementation, after the timeout, the system will seamlessly continue the consensus using the new topology. Thus, the vast majority of the reconfiguration time is spent awaiting the timeout of the current consensus instance.
In practise this timeout value represents a reasonable upper limit a consensus instance might need to terminate. Thus, it also highly correlates with the throughput of the system.

==> older-versions/evaluation-202101081820.tex <==
\section{Evaluation}
\label{sec:evaluation}

In this section we evaluate the performance of \thesystem in comparison with HotStuff. More specifically we:

\begin{enumerate}
    \item Assess the performance of different cryptographic operations to establish a baseline;
    \item Evaluate how \thesystem performs with regard to HotStuff;
    \item Evaluate the impact of the pipelining.
\end{enumerate}

\subsection{Setup}

We have used deployment sizes of $100, 200$ and $400$ processes and a fixed depth of $h=3$. Note that, with this number of nodes, we cannot achieve perfect $m$-ary trees. We explicitly avoided to used perfectly balanced trees in our evaluations as we consider this to be the most realistic scenario in practice. Thus, in our deployments, nodes are equally distributed down the tree to approximate a balanced tree. In all deployments we have fixed the depth of the tree to a value of $h=3$ and have adjusted the fanout $m$ of the root to maximize the pipelining depth. This resulted in different fanouts for each system size, namely, a fanout of  10 for 100 processes, a fanout of 20 for 200 processes (in this case, inner nodes have a smaller fanout, in the range of $[15,20]$), and a fanout of 20 for 400 processes.

All experiments presented in this paper were performed on the Grid'5000 testbed, supported by a scientific interest group hosted by Inria and including CNRS, RENATER and several Universities as well as other organizations~\cite{grid5000}. Each of the physical machines runs on two Intel Xeon E5-2620 v4 8-core CPUs with 64 GiB RAM. We've reserved up to 12 physical machines and, thus to scale the experimental setting, co-located always around 40 consensus processes. The center node of the star and the root node of the tree ran on separate physical machines individually. In order to avoid short communication paths within a physical machine, nodes ran on separate machines than their respective children and parents.

In order to simulate bandwidth and latency restrictions we used the native \textit{netem} tool on linux. We've restricted the latency at each individual machine and the bandwidth at the root/center process. We've considered a total of three different latency/bandwidth scenarios we've picked from the literature and actual use-cases. The first scenario is the use-case of a globally distributed blockchain similarly as proposed in \cite{motor, algorand, byzcoin} with $200ms$ roundtrip latency and $25Mb/s$ bandwidth. The remaining use-cases were picked from industry use-case scenarios reported in \cite{blockchain50}. Based on this, the next scenarios assume a reduced geographical distribution, for example for local supply-chain management, exchange of medical data, or digital currency (E-Euro, or E-Dollar). First, we got an US or EU wide scenario with a max of $100ms$ latency and $100Mb/s$ bandwidth and finally we got one country-wide (Germany, France, GB, etc) scenarios with $20ms$ roundtrip latency and $100Mb/s$ bandwidth. Similarly to most scenarios used in~\cite{yin2019hotstuff}, each block consists of $400$ operations resulting in a combined size of $100Kb$.

In the evaluation we focus on large-scale scenarios, where nodes are placed in different geographic locations and operate under bandwidth constraints. These scenarios are significantly different than the scenarios used for the evaluation of HotStuff in~\cite{yin2019hotstuff}, that considered a network latency of $1ms$ and the available bandwidth up to $8Gb/s$.

%Due to those restrictions, the results presented below show a significantly lower throughput than the results reported in the original \textit{HotStuff} paper~\cite{yin2019hotstuff}. This is the case since in the original experiments in \cite{yin2019hotstuff} the latency between the processes was $1ms$ and the measured bandwidth usage reached peaks of over $8Gb/s$ with $128$ processes. 

\subsection{Effect of Cryptographic Operations in the Busy Time}

As we have discussed in Section~\ref{sec:pipelining}, the maximum throughput of the system is limited by the Busy Time at the root, i.e., the time the root takes to send a block to its children, plus the additional time $\phi$ it requires to process the replies. Note that, in practice, communication and computation can partially overlap, that the formula $\textit{BT} = \frac{mB}{b}+\phi$ just provides an approximation. In system with low bandwidth \textit{BT} will be dominated by the communication, and in systems with low processing power it may be dominated by $\phi$. We now experimentally evaluate the values of $\phi$ for different cryptographic functions and different fanouts.

\thesystem uses \textit{bls-signatures}~\cite{bls,chia}. In this section we compare the compuation cost of bls operations with with \textit{secp} and with \textit{gpg}~\cite{gnupg}, which is the most common cryptographic library shipped with linux. Figure~\ref{fig:cryptocost} outlines the result of this experiment. Since \textit{bls-signatures} is based on cryptographic pairings, executing multiple verifications in sequence reduces the time to approximately $3400 us$ (over 5 operations). \textit{Bls-signatures} also come with an aggregation cost for both signatures and public keys (to verify aggregates). Similarly, due to the pairing based operations, aggregating larger numbers of elements reduces the time per element. The exact numbers for this are displayed in Figure~\ref{fig:blsagg}.

Table~\ref{table:phi} shows the resulting values for the processing time at the root $\phi$ for both HotStuff and \thesystem, for the configurations that we use in the implementations. The values for the computational cost $\phi$ were measured at the root node. As may be observed, Kauri scales inherently better, both in regards to its computational cost as well as in terms of bandwidth consumption. This allows us to leverage pipelining efficiently by using the spare computational power during the idle transmission times.

\begin{figure}
\begin{center}
\begin{subfigure}{0.33\textwidth}
    \centering \includegraphics[width=\textwidth]{figures/crypto.pdf}
	\caption{Single operation}
  \label{fig:crypto}
\end{subfigure}
\begin{subfigure}{0.33\textwidth}
     \centering\includegraphics[width=\textwidth]{figures/blsagg.pdf}
	\caption{Aggregation}
  \label{fig:blsagg}
\end{subfigure}
\end{center}
\caption{Cost of cryptographic operations (Sign and Verify)}
\label{fig:cryptocost}
\end{figure}

\begin{table}
\begin{center}
{\scriptsize
\begin{tabular}{l|r|r|r|r|r|r|r|r}
\hline
& \multicolumn{4}{c|}{HotStuff} & \multicolumn{4}{c}{\thesystem} \\\cline{2-9}
 & root  & &  &  & root  &  &  &  \\
\#nodes & fanout & $\phi$ & $\frac{mB}{b}$ & \textit{BT} & fanout & $\phi$ & $\frac{mB}{b}$ & \textit{BT} \\\hline
100     & 99  & 63,5 & 105,6 & 170.1 & 10 & 191,9 & 10,2 & 202,1\\
200     & 199 & 118 & 220,7 &  338.7& 20 & 224 & 20,5 & 244,5 \\
400     & 399 & 221,5 & 476,7 & 698,2 & 20 & 227,4 & 20,5 & 247,9 \\\hline
\end{tabular}
}
\end{center}
\caption{Values of $\phi$ for different scenarios in \textit{ms}}
\label{table:phi}
\end{table}

\subsection{Pipelining}
 
We now show the effect of pipelining and compare the observed behaviour with the behaviour predicted by our simplified performance model. For this experiment, we have chosen a scenario with $200ms$ roundtrip time and $25Mbit/s$ bandwidth. There is a total of $100$ processes, and the tree uses a fan-out of $10$. The block size $100kbit$.

For this configuration, the maximum speedup over HotStuff, when considering the bandwidth limitation alone is 10x. However, when the values of $\phi$ are taken into consideration, the Busy Time increases significantly. In our experiments, for this configuration of \thesystem, the observed value of $BT$ is approx 202. This means we cannot expect the implementation to achieve speedups larger than 5. However, since some parts of the computation can me multi-threaded, in a multi-threaded environment higher speedup factors might be possible.

\begin{figure}
\begin{center}
	\includegraphics[width=0.7\columnwidth]{figures/pipelining.pdf}
\end{center}
\caption{Pipelining}
\label{fig:figpiperes}
\end{figure}

In fact, as shown in Figure~\ref{fig:figpiperes}, we were able to scale the system up to 6 pipelined blocks. It was not possible to increase this further since the performance bonus of cryptographic pairings is lost with smaller numbers of sequentially evaluated signatures.

\subsection{Throughput}


We assess the performance of \thesystem in all three scenarios both with and without pipelining and compare it to the performance of HotStuff (with bls signatures and secp).
Figures \ref{fig:scenA}, \ref{fig:scenB}, \ref{fig:ScenC} contains the results of this experiment. While HotStuff offers better performance in runs with low numbers of processes, with increasing number of processes this dwindles and eventually \thesystem takes over.
This is the case since with low numbers of processes the latency induced cost of the tree based protocol is larger than the bandwidth and computing bottleneck of the star. However, with increasing numbers of processes this eventually shifts.


\begin{figure*}
	\centering
	\subfloat[$100ms$ latency and $100Mbit/s$ bandwidth\label{fig:scenA}]{\includegraphics[width=0.3\linewidth, height=3cm]{figures/A.pdf}}
	\subfloat[$100ms$ latency and $25Mbit/s$ bandwidth\label{fig:scenB}]{\includegraphics[width=0.3\linewidth, height=3cm]{figures/B.pdf}}
	\subfloat[$20ms$ latency and $100Mbit/s$ bandwidth\label{fig:scenC}]{\includegraphics[width=0.3\linewidth, height=3cm]{figures/C.pdf}}
	\caption{Throughput for different configurations.}
	\label{fig:throughput}
\end{figure*}



\begin{figure}[!htb]
     \centering
	\includegraphics[width=0.75\columnwidth, height=3cm]{figures/A.pdf}
	\caption{Throughput with 100ms and 100Mbit/s}
  \label{fig:scenA}
\end{figure}

\begin{figure}[!htb]
     \centering
	\includegraphics[width=0.75\columnwidth, height=3cm]{figures/B.pdf}
	\caption{Throughput with 200ms and 25Mbit/s}
  \label{fig:scenB}
\end{figure}

\begin{figure}[!htb]
     \centering
	\includegraphics[width=0.75\columnwidth, height=3cm]{figures/C.pdf}
	\caption{Throughput with 20ms and 100Mbit/s}
  \label{fig:ScenC}
\end{figure}


Using pipelining (Kauri (P)), in all three experiments, as shown in Figures \ref{fig:scenA}, \ref{fig:scenB}, \ref{fig:ScenC}, the throughput of \thesystem is significantly higher than the throughput of the star (independently if the star uses \textit{secp} or \textit{bls-signatures}).

As outlined before, in all scenarios, due to the large number of processes, the star bottlenecks at the bandwidth, significantly limiting its scalability. We may also observe this from the fact that the implementation of the star that uses \textit{bls-signatures} outperforms the one using \textit{secp} even though the computational cost is significantly higher. This is the case since \textit{secp} adds an additional strain on the bandwidth due to the requirement to disseminate $2f+1$ signatures each communication round.

Meanwhile, \thesystem leverages pipelining to compensate for the higher latency cost allowing it to produce a large number of blocks per second where both the computational as well as bandwidth consumption are equally distributed over the tree.

\subsection{Leader Replacement}

\begin{figure}
\begin{center}
	\includegraphics[width=0.7\columnwidth]{figures/recovery.pdf}
\end{center}
\caption{Reconfiguration after Failure}
\label{fig:reconfig}
\end{figure}

Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat, sed diam voluptua.

%todo: desc

\begin{figure}
\begin{center}
	\includegraphics[width=0.7\columnwidth]{figures/recovery.pdf}
\end{center}
\caption{Reconfiguration after Failure}
\label{fig:reconfig}
\end{figure}

Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat, sed diam voluptua. At vero eos et accusam et justo duo dolores et ea rebum. Stet clita kasd gubergren, no sea takimata sanctus est Lorem ipsum dolor sit amet. Lorem ipsum dolor sit amet, consetetur sadipscing elitr, sed diam nonumy eirmod tempor invidunt ut labore et dolore magna aliquyam erat, sed diam voluptua.

==> older-versions/evaluation-202101121150.tex <==
\section{Evaluation}
\label{sec:evaluation}

In this section, we evaluate the performance of \thesystem in comparison to HotStuff. 
We assess the following: i) performance comparison of the different cryptographic schemes to establish a baseline; ii)  comparison between \thesystem and HotStuff performance; iii) impact of the pipelining; and iv) the reconfiguration time. 

\subsection{Experimental Setup}

We use three system sizes with $N={100, 200, 300}$ processes and a fixed tree height $h=3$.
Rather than using some $N$ that yields perfect $m$-ary trees, which is unlikely in a real deployment, we use instead the system sizes above and distribute nodes to approximate a balanced tree as follows:
%Note that, with this number of nodes, we cannot achieve perfect $m$-ary trees. We explicitly avoided using perfectly balanced trees in our evaluations as we consider this to be an unrealistic scenario in practice. Thus, in our deployments, nodes are equally distributed down the tree to approximate a balanced tree. 
%We adjusted the fanout $m$ of the root to maximize the throughput. This resulted in different fanouts for each system size, 
for $N=100$, $m=10$ for the root and $m=[8,9]$ for the other interior nodes; for $N=200$ the root's fanout is $m=15$, and for the other interior nodes $m=[12,13]$, and for $N=400$, $m=20$ for the root and $m=[18,19]$ for the remaining interior nodes.
%mnamely, a fanout of  10 for 100 processes, a fanout of 20 for 200 processes (in this case, inner nodes have a smaller fanout, in the range of $[15,20]$), and a fanout of 20 for 400 processes.

All experiments were performed on the Grid'5000 testbed~\cite{grid5000}.
%, supported by a scientific interest group hosted by Inria and including CNRS, RENATER and several Universities as well as other organizations. 
Each machine has two Intel Xeon E5-2620 v4 8-core CPUs with 64 GB RAM. We used a total of 12 physical machines and evenly distribute the processes across the machines with the following rsetrictions: i) the leader always runs on a dedicated machine without any other process and ii) children and parent processes are always in different machines.
%, thus to scale the experimental setting, co-located always around 40 consensus processes. The center node of the star and the root node of the tree ran on separate physical machines individually. In order to avoid short communication paths within a physical machine, nodes ran on separate machines than their respective child and parent processes.
Besides processing capacity, network capacity also plays a key role in system performance.
To model the network characteristics, we use Linux's \textit{netem} to restrict bandwidth and latency among processes according to three different scenarios used in previous work and real uses-cases.
%We've restricted the latency at each individual machine and the bandwidth at the root/center process. We've considered a total of three different latency/bandwidth scenarios we've picked from the literature and actual use-cases. 

We consider three different deployments, namely the \textit{large-scale} deployment, the \textit{regional} deployment, and the  \textit{national} deployment.
The \textit{large-scale} deployment models a globally distributed blockchain as used in other works~\cite{motor, algorand, byzcoin} with $200ms$ roundtrip latency and $25Mb/s$ bandwidth.  The two other scenarios model reported industry use-cases~\cite{blockchain50}, in more limited geographical deployments for example for local supply-chain management, exchange of medical data, or digital currency (E-Euro, or E-Dollar).
The \textit{regional} deployment, captures a deployment in a large country or unions of countries, such as US or the EU, with $100ms$ roundtrip latency and $100Mb/s$ bandwidth.
Finally, the \textit{national} deployment models a setting where nodes are closer to each other, connected by a network  with $20ms$ roundtrip time and $100Mb/s$ bandwidth. 

We use a block size of $100Kb$, containing $400$ operations, as used for most scenarios in the original HotStuff's evaluation\cite{yin2019hotstuff}.
%, each block consists of $400$ operations resulting in a combined size of $100Kb$.
Note however that our work addresses geo-distributed deployments, which are significantly different than the local datacenter scenarios considered in~\cite{yin2019hotstuff}, that have a $1ms$ roundtrip latency and up to $8Gb/s$ of bandwidth usage.

%Due to those restrictions, the results presented below show a significantly lower throughput than the results reported in the original \textit{HotStuff} paper~\cite{yin2019hotstuff}. This is the case since in the original experiments in \cite{yin2019hotstuff} the latency between the processes was $1ms$ and the measured bandwidth usage reached peaks of over $8Gb/s$ with $128$ processes. 

\subsection{Effect of Cryptographic Operations in the Busy Time}

As discussed in Section~\ref{sec:pipelining}, the system throughput is limited by the Busy Time at the root, \emph{i.e.}, the time the root takes to send a block to its children, plus the additional time $\phi$ it requires to process the replies. Note that, in practice, communication and computation can partially overlap, and thus $\textit{BT} = \frac{mB}{b}+\phi$  provides just an approximation. In system with low bandwidth, \textit{BT} will be dominated by the communication, and in systems with low processing power it may be dominated by $\phi$. Next, we evaluate the values of $\phi$ for different  cryptographic schemes: i) \textit{secp256k1} used by HotStuff, ii) \textit{bls}~\cite{bls,chia} used by \thesystem
 and iii) \textit{gpg}~\cite{gnupg}, a classic cryptographic scheme.

% \textit{bls-signatures}~\cite{bls,chia}. Next, we compare the compuation cost of bls operations with with \textit{secp} and with \textit{gpg}~\cite{gnupg}, which is the most common cryptographic library shipped with linux.
Figure~\ref{fig:crypto} shows the cost of a single sign and verify operation averaged over 5 runs for each scheme.
As one can see, \textit{gpg} is substantially slower than \textit{bls} and \textit{secp256k1}, with the latter clearly outperforming \textit{bls}.
However, while the cost of \textit{gpg} and \textit{secp256k1} grows linearly with the number of signatures, \textit{bls} amortizes this cost through aggregation. 
The results for \textit{bls} aggregation are show in Figure~\ref{fig:blsagg} and can be decomposed in aggregation of the public keys to create an aggregated public key, and verification of the aggregated signatures using that key.
Interestingly the aggregation cost decreases quickly with the number of signatures and the verification cost is constant (Figure~\ref{fig:crypto}).
In contrast, the verification cost of the other schemes is linear with the number of signatures.
This means that after $\approx 55$ signatures (\emph{i.e.} inputs of processes), the overall cost of \textit{secp256k1} surpasses that of \textit{bls}.


%outlines the result of this experiment. Since \textit{bls-signatures} is based on cryptographic pairings, executing multiple verifications in sequence reduces the time to approximately $3400 us$ (over 5 operations). \textit{Bls-signatures} also come with an aggregation cost for both signatures and public keys (to verify aggregates). Similarly, due to the pairing based operations, aggregating larger numbers of elements reduces the per element time. The exact numbers for this are displayed in Figure~\ref{fig:blsagg}.

We use these values to estimate the $\phi$ and computational and communication speedup for different system sizes in the \textit{global} deployment, as shown in Table~\ref{table:phi}. %shows the resulting values for the processing time at the root $\phi$ for both HotStuff and \thesystem, at  The values for the computational cost $\phi$ were measured at the root node. 
As may be observed,  while \thesystem has a higher base computational cost $\phi$ due to the \textit{bls} scheme, it scales inherently better than HotStuff which relies on \textit{secp256k1}, %This results in \thesystem providing better potential communication and computational speedups by    
and provides better speedups in terms both in terms of its computational cost as well as in terms of bandwidth consumption. This allows us to leverage pipelining efficiently by using the spare computational power during the idle transmission times.

\begin{figure}
	\centering
	\subfloat[Single operation\label{fig:crypto}]{\includegraphics[width=0.49\linewidth]{figures/crypto.pdf}}\,
	\subfloat[\textit{bls} Aggregation\label{fig:blsagg}]{\includegraphics[width=0.49\linewidth]{figures/blsagg.pdf}}
    \caption{Cost of cryptographic operations (Sign and Verify)}
    \label{fig:cryptocost}
\end{figure}


%\begin{table}
%\begin{center}
%{\scriptsize
%\begin{tabular}{l|r|r|r|r|r|r|r|r}
%%\hline
%& \multicolumn{4}{c|}{HotStuff} & %\multicolumn{4}{c}{\thesystem} \\\cline{2-9}
% & root  & &  &  & root  &  &  &  \\
%\#nodes & fanout & $\phi$ & $\frac{mB}{b}$ & \textit{BT} & fanout & $\phi$ & $\frac{mB}{b}$ & \textit{BT} \\\hline
%100     & 99  & 63,5 & 422 & 485,5 & 10 & 191,9 & 4,1 & 196\\
%200     & 199 & 118 & 883 & 1001 & 20 & 224 & 8,2 & 232,2 \\
%400     & 399 & 221,5 & 1907 & 2128,5 & 20 & 227,4 & 8,2 & 235,6 \\\hline
%\end{tabular}
%}
%\end{center}
%\caption{Values of $\phi$ for different scenarios in %\textit{ms}}
%\label{table:phi}
%\end{table}

\begin{table}
\begin{center}
{\scriptsize
\begin{tabular}{l|r|r|r|r|r|r}
\hline
& \multicolumn{6}{c}{HotStuff }  \\ \hline
 & root  & &  &  & max depth &  max depth \\
\#nodes & fanout & $\phi$ (ms) & $\frac{mB}{b}$ & \textit{BT} & (comm.) & (cpu) \\\hline
100     & 99  & 63,5 & 550,0 & 613,5 & 0,36 & 15,75 \\
200     & 199 & 118,0 & 1375,4 & 1493,4 & 0,14 & 8,47  \\
400     & 399 & 221,5 & 3843,3 & 4064,8 & 0,05 & 4,51 \\\hline

& \multicolumn{6}{c}{\thesystem} \\ \hline
100       & 10 & 191,9 & 41,7 & 196 & 9,59 & 5,20\\
200       & 20 & 224,0 & 83,4 & 232,2 & 4,8 & 4,46\\
400       & 20 & 227,4 & 83,4 & 235,6 & 4,8 & 4,40\\\hline


\end{tabular}
}
\end{center}
\caption{Pipelining detpth for the \textit{large-scale} deployment with different system sizes.}
\label{table:phi}
\end{table}

\subsection{Pipelining}
 
We now show the effect of pipelining and compare the observed behaviour with the behaviour predicted by our simplified performance model on the \textit{large-scale} deployment ($200ms$ latency  and $25Mbit/s$ bandwidth) with $100$ processes.
%. There is a total of $100$ processes, and the tree uses a fan-out of $10$. 

For this configuration, as shown in Table~\ref{tab:examples}, when considering the bandwidth limitation alone, the maximum speedup over HotStuff is 10x. However, from Table~\ref{table:phi},  it is possible to see that this configuration is cpu-bounded and that, given that $\phi \approx 190$, the  expected speedup should not be much larger than 5. In fact, as shown in Figure~\ref{fig:figpiperes}, we were able to scale the system up to 6 pipelined blocks almost linearly, benefiting from some  overlap between transmission and computation time. 

\begin{figure}
\begin{center}
	\includegraphics[width=0.7\columnwidth]{figures/pipelining.pdf}
\end{center}
\caption{Pipelining with increasing depth levels}
\label{fig:figpiperes}
\end{figure}

%In fact, as shown in Figure~\ref{fig:figpiperes}, we were able to scale the system up to 6 pipelined blocks almost linearly.
%It was not possible to increase this further since the performance bonus of cryptographic pairings is lost with smaller numbers of sequentially evaluated signatures.

\subsection{Throughput}


Next, we assess the performance of \thesystem  both with pipelining (\thesystemfull) and without pipelining (\thesystemcrippled) and compare it to the performance of HotStuff with bls signatures (HotSuff-bls)  and secp (HotStuff-secp). Figures~\ref{fig:scenA}, \ref{fig:scenB}, and~\ref{fig:scenC} contain the results of this experiment. While HotStuff offers better performance in runs with low numbers of processes, compared to \thesystemcrippled, with increasing numbers of processes this dwindles and eventually \thesystem takes over. This is the case since with low numbers of processes the latency induced cost of the tree based protocol is larger than the bandwidth and computing bottleneck of the star. However, with increasing numbers of processes this eventually shifts.


\begin{figure*}[t]
	\centering
	\subfloat[large-scale ($200ms-25Mb/s$)\label{fig:scenB}]{\includegraphics[width=0.3\linewidth, height=3cm]{figures/B.pdf}}\,\,\,
	\subfloat[regional ($100ms-100Mb/s$)\label{fig:scenA}]{\includegraphics[width=0.3\linewidth, height=3cm]{figures/A.pdf}}\,\,\,
	\subfloat[national ($20ms-100Mb/s$)\label{fig:scenC}]{\includegraphics[width=0.3\linewidth, height=3cm]{figures/C.pdf}}
	\caption{Throughput for different latency/throughput configurations.}
	\label{fig:throughput}
\end{figure*}


In all three experiments, as shown in Figures~\ref{fig:scenA}, \ref{fig:scenB}, and~\ref{fig:scenC}, the throughput of \thesystemfull is significantly higher than the throughput of both HotStuff-bls and HotStuff-secp.  As outlined before, in all scenarios, due to the large number of processes, the star bottlenecks at the bandwidth, significantly limiting its scalability. We may also observe this from the fact that the implementation of the star that uses \textit{bls-signatures} outperforms the one using \textit{secp} even though the computational cost is significantly higher. This is the case since \textit{secp} adds an additional strain on the bandwidth due to the requirement to disseminate $2f+1$ signatures each communication round. This way, while \thesystemfull offers up to 17x the throughput of HotStuff-bls, it beats the native HotStuff implementation by a factor of 38.

Also, \thesystemfull leverages pipelining to compensate for the higher latency cost allowing it to produce a large number of blocks per second where both the computational as well as bandwidth consumption are equally distributed over the tree.

\subsection{Leader Replacement}

Finally, we evaluate how \thesystem compares in terms of reconfiguration performance. For this purposed we have injected faults in the system to force one or more reconfigurations. In the both cases the current leader fails, but in one case, the next leader is correct and, in the other case, the next two  leaders are also faulty. For both Kauri and HotSuff we have experimentally computed that lowest timeout possible that would not lead to spurious reconfigurations in steady-state. This resulted in a timeout value of $0.3ms$ for \thesystem and $0.75ms$ for HotStuff. The results of those experiments are depicted in Figure~\ref{fig:reconfig}. The results show that \thesystem recovers quickly from the injected fault.  Also, shortly after recovery,  the pipelining is filled again, bringing the system back to the original throughput.

\begin{figure}[t]
	\centering
	\subfloat[1 fault\label{fig:reconfig1}]{\includegraphics[width=0.48\columnwidth]{figures/reconfig.pdf}}\,
	\subfloat[3 simultaneous faults\label{fig:reconfig2}]{\includegraphics[width=0.48\columnwidth]{figures/reconf3.pdf}}
	\caption{Reconfiguration after Failure}
\label{fig:reconfig}
\end{figure}

 

==> older-versions/intro-202011061420.tex <==
\section{Introduction}

Blockchains such as Bitcoin~\cite{bitcoin} or Ethereum~\cite{ethereum} are permissionless, i.e., they do not impose constraints on the number of nodes that may participate in consensus. They use randomized consensus protocols inspired by the \emph{Nakamoto consensus}~\cite{bitcoin}, that suffers from the well-known problem of allowing forks in blockchain, which eventually causes some already committed transaction to be aborted. Further, permissionless consensus protocols are unable to offer high throughput\cite{xx,yy}.

As the range of application of blockchains expands to  enterprise and government areas, permissioned blockchains, such as Hyperledger Fabric~\cite{HyperledgerBlockchain}, have gained an increasing attention. Because the number of participants is bound and known, it is possible to run consensus algorithms that provide finality. Also, these algorithms can offer much higher throughput than their permissionless counterparts\cite{PoWVsBft}.

Permissioned blockchains rely on variants of classical byzantine fault-tolerant consensus protocols\cite{dls,lamport}, which are difficult to scale for very-large number of participants. However, settings with number of participants as high as XXX and YYY are common in existing blockchains\cite{xx,yy}. The scalability issues derive from the high number of messages that need to be exchanged and processed to reach consensus. PBFT\cite{pbft} organizes participants in a clique and has a quadratic message complexity. More recent algorithms, such as HotStuff\cite{hotstuff}, organize participants in a star topology, which allows to reduce the message complexity but fails to reduce the load on the coordinator, that is still required to receive and validate votes from all other processes. These algorithms are, therefore, inherently non-scalable. These limitations have raised an increasing interest in finding techniques that can make byzantine fault-tolerant consensus scale~\cite{byzcoin,Motor}.

An effective strategy to distribute the load, and therefore increase the scalability of the system, consists in organizing the participants in a logical tree, that can be used by the leader both to aggregate votes and to disseminate the result. By using cryptographic tools such as XXX\cite{xxx} and YYY\cite{yyy},  a node in the tree can aggregate the votes of its children. This allows global aggregation to performed cooperatively and in parallel, as votes are propagated to the leader. Then, the leader can validate the aggregation, a step that can be implemented more efficiently than the process of validating every individual vote, as performed by protocols such as HotStuff. Systems such as \textit{Byzcoin}~\cite{byzcoin} or \textit{Motor}~\cite{Motor} propose using a tree topology to distribute the load of verification and aggregation among the participating processes.

The use of aggregation trees in this context does raise, however, serious challenges, as it makes  the consensus less robust: a faulty interior node may prevent aggregation to terminate. More importantly, in many cases, finding a tree that does not include faulty-inner nodes may require a number of reconfigurations that is factorial with the system size. This contrasts with algorithms based on a clique or a start, that can terminate after $t+1$ reconfigurations.  Due to this problem, to the best of our knowledge, previous algorithms that explore the use of trees to aggregate votes always fall back in faulty-runs to non-scalable topologies, such as a clique or a star.  

In this paper we propose \thesystem, the first BFT consensus protocol that organizes participants in a tree to perform scalable vote aggregation while still converging to a (tree-based) robust configuration in optimal number of steps $\mathcal{O}(t)$.  We define precisely which aggregation trees allow for optimal reconfiguration and discuss the tradeoffs among the resilience, the fanout of the tree, and the number of reconfigurations required to ensure termination.

To maximize the amount of parallelisation made possible by the use of an aggregation tree, \thesystem uses a pipelining scheme that allows nodes at different depths of the tree to aggregate in parallel votes for different consensus instances.  This pipelining scheme allows to increase the throughput of the system by a factor of XXX with regard to a non-pipelined version.

We have implemented \thesystem and evaluated the resulting system experimentally on different settings. Our results show that  \thesystem can outperform HotStuff in settings up to XXX participants. THIS NEEDS TO BE IMPROVED.

\textbf{Luis: I am at this point}

While permissionless blockchains like Bitcoin or Ethereum~\cite{bitcoin, ethereum} have received significant attention, permissioned blockchains such as Hyperledger Fabric~\cite{HyperledgerBlockchain} are playing an ever increasing role in diverse enterprise and government use-cases.

Permissioned blockchains limit the group of participants that are allowed to participate in consensus. Because the number of participants is bound and known, it is possible to run consensus algorithms that provide finality and thus avoid the well-known problem of forks in blockchains based on the so-called \emph{Nakamoto consensus}~\cite{bitcoin}. Not only that, these algorithms are known to offer much higher throughput than their permissionless counterparts \cite{PoWVsBft}.

These algorithms are typically inspired by classical Byzantine consensus algorithms, such as PBFT~\cite{pbft}. PBFT organizes processes in a clique topology and uses an all-to-all communication pattern. While this offers robustness under faults, it also results in a quadratic message complexity which has a negative impact on scalability. Therefore, recent works have proposed alternative topologies with the goal of reducing message complexity and distributing the load among participants.

For instance, \textit{HotStuff}~\cite{hotstuff} organizes processes in a star topology, where the process that is placed at the center of the star plays the role of the leader: processes send the information to the leader that, in turn, sends back aggregated results to the other processes. 

However, having the central process verify and aggregate $\mathcal{O}(n)$ signatures quickly leads to a performance bottleneck.

Therefore, approaches like \textit{Byzcoin}~\cite{byzcoin} or \textit{Motor}~\cite{Motor} propose using a tree topology to distribute the load of verification and aggregation among the participating processes.

Note that when moving from a clique to a less robust topology the impact of faults is magnified, in particular if these happen at the central node of a star topology or at the root or internal nodes of a tree topology.

Thus, efficient reconfiguration strategies are necessary to select correct nodes for these important positions in the topology.
For instance, consider \textit{HotStuff} which leverages a star topology, where the leader is the process located in the center of the star. Even using a naive reconfiguration strategy, the leader in the center of the star is guaranteed to be a correct process after at most $f+1$ steps. However, for trees replacing the root is not enough as faulty internal nodes can still disrupt the communication.

In fact, previous works note that tree reconfiguration requires an exponential number of steps~\cite{Motor}. To overcome these, a number of optimistic algorithms rely on a less robust communication pattern in the ``good'' case, and fall back to an all-to-all communication pattern when consensus fails to terminate~\cite{byzcoin}. On the other hand, the remaining algorithms that do not require an immediate fall-back to a clique or star restrict the topology to a two level hierarchy and still fall back slowly to a star topology.

Not only that, none of these approaches actually compare their performance to high throughput solutions as \textit{Hotstuff}.

In this paper we propose \thesystem, a high throughput tree based byzantine fault tolerance consensus protocol that supports arbitrary trees and offers a novel reconfiguration strategy and avoids immediate fall-back to a star or clique.

We show that our solution not only scales significantly better than \textit{HotStuff} but also that we can outperform \textit{HotStuff} in many realistic scenarios.

In short, the paper makes the following contributions:

\begin{itemize}

\item We present \thesystem a tree based BFT consensus algorithm;
\item We present a novel reconfiguration strategy that works for arbitrary trees;
\item We experimentally and mathematically show the scalability and performance advantage of our approach over state of the art approaches. 

\end{itemize}

The rest of this paper is organized as follows. First, in Section~\ref{sec:relatedwork} we discuss the related work and how our approach compares to algorithms in the literature. Next, Section~\ref{sec:model} describes the considered system model. Following that, in Section~\ref{sec:thesystem} we present the details of our approach. Based on that, Section~\ref{sec:implementation} discussed the prototype and Section~\ref{sec:evaluation} the evaluation and discussion of the obtained results. Finally, Section~\ref{sec:conclusions} concludes the paper.


==> older-versions/intro-202012211515.tex <==
\section{Introduction}

%\ray{I think we should scrap the following paragraph entirely.}
%The popularity of permissionless blockchains such as Bitcoin\cite{bitcoin} or Ethereum\cite{ethereum} stems from the fact that anyone can participate in the system. Such systems are supported by Sybil-resistant randomized consensus protocols inspired by the \emph{Nakamoto consensus} first proposed in Bitcoin\cite{bitcoin}. While the permissionless characteristics are attractive and can support thousands of participants, these protocols suffer from two major shortcomings: i) forks, which prevents applications from determining whether a transaction is committed or not, a property also known as finality and ii) very low throughput, in the order of a few dozens transactions per second\cite{PoWVsBft}.

As the range of blockchain applications expands to enterprise and government areas, permissioned blockchains, such as Hyperledger Fabric\cite{HyperledgerBlockchain}, have gained increasing attention. 
By having a restricted and well-known number of participants, permissioned blockchains can employ classical consensus protocols which bring two main advantages over permissionless approaches: transaction finality and high throughput\cite{PoWVsBft}.
%in the protocol ecause the number of participants is bound and known, it is possible to run classical consensus algorithms that provide finality. Also, these algorithms can offer much higher throughput than their permissionless counterparts

There is a strong demand for permissioned blockchains able to scale up to a thousand participants~\cite{sbft}, as Diem (formerly Libra) pointed out in their whitepaper: "Our goal was to choose a protocol that would initially support at least 100 validators and would be able to evolve over time to support 500–1,000 validators."~\cite{libradocs}.

However, the classical byzantine fault-tolerant consensus protocols those systems currently hinge on scale poorly with the number of participants\cite{dls,byzGens}.
%, which are difficult to scale for very-large number of participants. 
These scalability issues derive from the high number of messages that need to be exchanged and processed to reach consensus. For instance, the well-known PBFT protocol\cite{pbft} organizes participants in a clique resulting in a quadratic message complexity. More recent algorithms, such as HotStuff\cite{hotstuff}, organize participants in a star topology, which allows to reduce the message complexity but fails to reduce the processing load on the coordinator, that is still required to receive and validate votes from all other processes. These algorithms are, therefore, inherently non-scalable. 

%These limitations have raised an increasing interest in finding techniques that can make byzantine fault-tolerant consensus scale\cite{byzcoin,motor}.

An effective strategy to distribute the load, and therefore increase the scalability of the system, consists in organizing the participants in a logical tree, that can be used by the leader both to aggregate votes and to disseminate the consensus result. 
By combining a tree topology with cryptographic schemes such as multi signatures\cite{byzcoin} or aggregated signatures\cite{bls}, a node in the tree can aggregate the votes of its children before propagating them to its parent. 
This allows votes to be collected and aggregated in parallel, as votes are propagated from the leaf to the leader at the root of the tree. 
These cryptographic schemes allow the leader to validate the aggregated votes at a fraction of the cost of validating each vote individually.
%Following that, the process at the root only has to validate the aggregation, a step that can be implemented more efficiently than the process of validating every individual vote, as performed by protocols such as HotStuff. 
This approach is explored by systems such as Byzcoin\cite{byzcoin} or Motor\cite{motor} that offer better load balancing properties than the centralized approach proposed by HotStuff. 
%propose using a tree topology to distribute the verification and aggregation load among the participating processes.

Note, however, that the use of trees inherently makes consensus less robust, as the failure of a single internal node may prevent aggregation from terminating.
In a system with a clique of star topology, such as PBFT or HotStuff, respectively, it is enough to perform $f+1$ reconfigurations to ensure termination (when the network is stable), for $f$ faulty nodes. When such a failure happens in a tree topology, it is necessary to find a tree where no internal node is faulty which may require an exponential number of steps with respect to the system size~\cite{motor}.
Note that, while the reconfiguration process takes place the system is essentially halted which has a significant negative impact on the applications.
%The use of aggregation trees in this context does raise, however, serious challenges, as it makes the consensus less robust: a faulty internal node may prevent aggregation to terminate. 
%More importantly, in many cases, finding a tree without any faulty internal nodes may require a number of reconfigurations that is exponential with the system size\cite{motor}. This contrasts with algorithms based on a clique or star, that can terminate after $f+1$ reconfigurations. 
To mitigate this problem, state of the art algorithms, upon failing to collect a quorum within a certain time, assume a faulty internal node and fall back to a clique or star topology\cite{byzcoin,motor}.
Moreover, upon falling back to such non scalable topologies, these approaches do not offer a deterministic strategy to construct a robust tree topology, and hence potentially stay in a degraded state indefinitely.
As in a large scale systems faults are the norm rather than the exception, it is thus very likely that any long term deployment will be in a degraded state with a substantial negative impact on the throughput which directly affects the applications. In Byzcoin, for example, a single faulty node has a 50\% chance of leading the system to a degraded state.

%Due to this problem, to the best of our knowledge, previous algorithms that explore the use of trees to aggregate votes always fall back in faulty-runs to non-scalable topologies, such as a clique or a star. On the top of that, none of these algorithms offer recovery strategies to eventually return to the original topology.

In this paper, we propose \thesystem, the first communication protocol for BFT consensus that organizes participants in a tree topology
and, upon failures, guarantees optimal reconfiguration, \emph{i.e.} in $f+1$ steps.
%to perform scalable vote aggregation while still converging to a (tree-based) robust configuration in an optimal number of steps $\mathcal{O}(t)$.  
We precisely define which trees allow optimal reconfiguration, and discuss the tradeoffs between resilience, the fan-out of the tree, and the number of reconfigurations required to ensure termination.

To maximize the amount of parallelisation made possible by the use of an aggregation tree, \thesystem uses a novel pipelining scheme that allows nodes at different depths of the tree to aggregate votes for different consensus instances in parallel. As we show in the evaluation, this pipelining scheme allows to increase the throughput of the system by up to 6 times when compared to the non-pipelined version.

We have implemented \thesystem and evaluated the resulting system experimentally on different settings. Our results show that \thesystem can outperform HotStuff in a range of different deployment scenarios with up to 400 processes. Thus, \thesystem provides a up to 17 times higher throughput than the throughput of HotStuff using the star topology.

In short, the paper makes the following contributions:

\begin{itemize}
\item We present a set of abstractions that support the use of aggregation/dissemination trees in the context of consensus protocols;
\item We present a precise characterization of trees that support optimal reconfiguration steps;
\item We present \thesystem,  the first consensus protocol based on aggregation-trees that reconfigures in optimal time;
\item We show how pipelining can be used to make full use of the parallelisation opportunities offered by the use of aggregation trees;
\item We present an extensive experimental evaluation of \thesystem with up to 400 nodes.

\end{itemize}

The rest of this paper is organized as follows. First, in Section~\ref{sec:relatedwork} we discuss the related work and how our approach compares to the state of the art. Section~\ref{sec:systemmodel} describes the system model and Section~\ref{sec:trees} starts outlining \thesystem.
Next, Section~\ref{sec:reconfiguration} and Section~\ref{sec:pipelining} describe how the proposed system deals with the drawbacks of tree structures.
Following that, Section~\ref{sec:implementation} describes the implementation of \thesystem that is evaluated in Section~\ref{sec:evaluation} and, finally, Section~\ref{sec:conclusion} concludes the paper.


==> older-versions/kauri-202011251826.tex <==
\section{Kauri}
\label{sec:thesystem}

In this section we present \thesystem. We start by introducing the \ldots

\subsection{Overview}
\label{sec:overview}

The design of \thesystem is centered around three main objectives: 
%The contributions of this paper are centered on the communication patterns used to convey information from participants to the leader and from the leader to the participants, such that the 
i) reduced message complexity, ii) load balancing and iii) upon failures, reconfiguration in a optimal number of steps.

%up is reduced, load balancing  is achieved, and reconfiguration in an optimal number of steps can still be performed. 

Rather than proposing a new consensus protocol from scratch, we focus instead on the communication patterns and reconfiguration process necessary to achieve the objectives above.


To simplify our presentation, we frame our contributions within the scope of \textit{HotStuff}, but our techniques are generic and can be used in other leader-based consensus algorithms.
We will also use the publicly available implementation of \textit{HotStuff} as a baseline later in our evaluation (Section~\ref{sec:evaluation}).
%The proposed techniques are general, and can potentially be applied to several consensus protocols. 

%To make the presentation concrete, and to perform an empirical evaluation, we have adopted an existing consensus algorithm and have introduced just the required changes such that it can operate with the newly proposed communication patterns. Namely, we depart from \textit{HotStuff}, that is based on a start topology.  

\textit{HotStuff} uses a star topology (Figure~\ref{fig:examplestar}) and requires three rounds of communication (Figure~\ref{fig:threephasehotstuf}). 
The objective of each round is to collect a quorum of signatures (votes) where each round consists of two steps: i )the leader sends some information to all other participants, and ii) the leader collects inputs from those participants. 
As discussed in Section~\ref{sec:relatedwork}, the leader needs to communicates directly with $N-1$ processes, and verify all the received inputs. Therefore, and as we show in the evaluation (Section~\ref{sec:evaluation}), the CPU and/or the bandwidth at the leader can easily become a bottleneck.

In \thesystem we change the star topology to a tree-based topology (Figure~\ref{fig:exampletree}) while still preserving the three communication rounds (Figure~\ref{fig:threephase}) and the overall properties of the consensus algorithm.

%Our implementation uses exactly the same structure, based on three rounds of communication as \textit{HotStuff}. However, in \thesystem we replace the start topology for a tree topology, as illustrated in Figures~\ref{fig:exampletree} and~\ref{fig:threephase}.
%Our consensus algorithm is an adjusted version of \textit{HotStuff} but instead of working on a star we leverage a tree topology. We, therefore, also assume a three phase protocol where in each phase a quorum of signatures has to be collected.

\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/threephase.pdf}
	\caption{Tree of depth 3}
  \label{fig:threephase}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/hotstuffalgo.pdf}
  \caption{Star}
  \label{fig:threephasehotstuf}
\end{subfigure}
\caption{Three Phase Protocol}
\label{fig:fig}
\end{figure}

%The three phase protocol is displayed in Figure~\ref{fig:threephase}.
Considering the simple tree topology depicted in Figure~\ref{fig:exampletree}, the leader process $P_0$ collects three quorums, distributes them to internal nodes $P_1, P_2, P_3$ which in turn relay them to leaf processes $L_1$ to $L_3$ (dotted lines).

The additional communication that is necessary is displayed using the dotted line. 
Note that this comes at an additional latency costs due to the relay from the inner processes to the leafs, however the distribution of the computational and bandwidth load yields substantial benefits at scale.
As we will see later, in certain scenarios it is even possible for the tree to provide better latency than the star based topology (Section~\mm{XXX, make sure we show this}).

%While this results in additional latency due to the additional communication steps it distributes the aggregation and verification overhead of the signatures over a set of processes to improve the scalability.

\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.4\textwidth]{figures/exampletree.pdf}
	\caption{Example Tree of depth 3}
  \label{fig:exampletree}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.4\textwidth]{figures/hotstuffstar.pdf}
  \caption{Star}
  \label{fig:examplestar}
\end{subfigure}
\caption{Communication Topologies}
\label{fig:fig}
\end{figure}

Since we follow the same general structure as \textit{HotStuff}, the safety properties of the algorithm apply directly to our approach\mm{this is too vague, we need a better discussion here, which can appear later in the paper}. 
However, due to the nature of a tree topology, ensuring liveness imposes an additional set of requirements and properties.
We define and discuss those requirements and properties in the next section.

%The respective tree that matches the protocol highlighted in Figure~\ref{fig:threephase} can be found in Figure~\ref{fig:exampletree}.
%With $P_0$ at the root, through the internal processes $P_i$ down to the leaf processes $L_i$.

%MM: this is fundamental to show, but I'm not sure this is the right place
%This way, safety is guaranteed as proven in \cite{hotstuff}. While most of the liveness proof also applies in this case, collecting signatures over a tree topology is inherently more complex than over a star. 
%This is the case, since even if the root is a correct process, faulty internal nodes may not relay all correct signatures.

\subsection{Properties and Definitions}

\begin{mod}
{\footnotesize
\textbf{Definitions:}
\begin{quote}
  \emph{Fault-Completeness:} A collection $c_{i}$ is denoted to be \textit{$f$-complete} if $|c_i| \geq N-f$.
\end{quote}
\begin{quote}
  \emph{Consistency:} Let process $p_i$ output collection $c_{i}$ and process $p_j$ output collection $c_{j}$ such that $(p_x, v_x)\in c_{i}$ and $(p_x, v'_x) \in c_{j}$. Collection $c_{i}$ and collection $c_{j}$ are \textit{consistent} iff $v_x = v'_x$.
\end{quote}
\begin{quote}
  \emph{Integrity:} Let collection $c_{i}$ be output at process $p_i$. Collection $c_{i}$ is said to fulfill \textit{integrity} iff, for every $(p_x, v_x) \in c_{i}$, $v_x$ was the value input by process $p_x$.
\end{quote}
\textbf{Properties:}
\begin{quote}
  \emph{Termination:} If a correct process $p_i$ inputs \textit{$(p_i, v_i)$} it eventually outputs $c_{i}$. 
\end{quote}
\begin{quote}
  \emph{Fulfillment:} The collection $c_{i}$ output at every correct processes satisfies $f$-completeness, consistency, and integrity.
\end{quote}
}
\caption{Communication abstraction}
\label{mod:tob}
\end{mod}

In order to support the proposed structure, we specify a set of properties that have to be fulfilled outlined in Abstraction~\ref{mod:tob}. 

Based on that, we identify the robustness of the communication topology to be the key requirement.

\begin{definition}
\textbf{Robust Graph:} An edge is said to be \textit{safe} if the corresponding vertices are both correct processes. A graph is robust iff for every pair of correct process $p_i$ and $p_j$, there is a path between $p_i$ and $p_j$ composed exclusively of safe edges. \label{def:robust}
\end{definition}

\begin{theorem}
\label{th:robust}
If the communication graph is not robust, fulfillment cannot be achieved.
\end{theorem}

\begin{proof}
For fulfillment to be achieved, $f$-completeness has to be observed. $f$-completeness requires that $N-f$ processes are able to contribute their value to the output collection. The proof is by contradiction. Assume there is a non-robust graph that achieves fulfillment and, thus, $f$-completeness. Assume a run where $f$ faulty processes do not produce any input and do not relay messages. To achieve $f$-completeness every correct process needs to collect the input from all other correct processes. However, as the graph is not robust, there is at least one pair of correct processes $p_i$ and $p_j$ without a communication path consisting of safe edges between them. This leads to a contradiction since an adversary can prevent these processes from exchanging their values, preventing $f$-completeness from being fulfilled.
\end{proof}


\paragraph*{Eventual Fulfillment}

It is well known that consensus protocols for asynchronous systems may not terminate while the system is in an asynchronous phase, and may need multiple rounds of communication until the system stabilizes. We denote the system during asynchronous phases as \textit{unstable} and otherwise \textit{stable}. Additionally, to ensure termination leader-based consensus protocols are required to change leader when the leader is deemed faulty. 

The termination of the communication primitive and the consensus algorithm are heavily intertwined as a non-robust communication topology might not allow the collection of sufficient quorums and, thus, it might not be possible for consensus to terminate. Additionally, in a non-robust topology, correct processes might not receive the result of a successful consensus and fail to terminate.

Therefore, to ensure consensus termination, the system must be stable and the communication graph must be robust. To ensure the latter, we need to iterate over a sequence $G_1, G_2, G_3, .., G_n$ of static graphs, which we denote as an evolving graph $\mathcal{G}$.

We say \textit{eventual fulfillment} is achieved iff there is a $k$ such that the communication on $G_k$ achieves fulfillment. As discussed previously, this cannot be guaranteed unless the system is stable \textit{and} the static graph $G_k$ is robust. Given the definition of a robust static graph, we can define a necessary condition that an evolving graph $\mathcal{G}$ needs to satisfy, such that eventual fulfillment may be provided:

\begin{definition} 
\textbf{Recurringly Robust Evolving Graph:} An evolving graph $\mathcal{G}$ is denoted to be \textit{recurringly robust} iff robust static graphs appear infinitely often in its sequence. \label{def:recurringlyrobust}
\end{definition}

\begin{theorem}
If the evolving graph is not recurringly robust,  eventual fulfillment cannot be guaranteed.
\end{theorem}

\begin{proof}
Following Theorem~\ref{th:robust}, fulfillment cannot be achieved if the graph is not robust. However, even a robust graph cannot guarantee fulfillment while the system is unstable. This happens because a correct process can not distinguish between a faulty process and a process that is slow\cite{flp}. This could lead to scenarios where processes wait indefinitely for answers of faulty processes. If there is only a finite number of robust graphs in the evolving graph, in an infinite sequence of static graphs,  all instances of robust graphs could occur during periods of instability. Therefore, robust graphs must appear infinitely often in the evolving graph.
\end{proof}

While this seems like a strong condition, this can be easily achieved with a reconfiguration strategy that terminates in finite steps and contains at least one robust graph. We later present  in Section~\ref{sec:conformity}, algorithms that fulfill these properties.

\paragraph*{$t$-Bounded Conformity and Optimal Conformity}

Although a recurringly robust evolving graph is sufficient to achieve eventual fulfillment, this condition does not guarantee an efficient implementation.
In fact, after the system becomes stable, a large number of reconfigurations may still be required to reach fulfillment. Ideally, when the system becomes stable, we would like to reach fulfillment after a small number $t$ of attempts, a property that we denote \textit{$t$-bounded conformity}. 
%We can define precisely the property an evolving graph must exhibit such that fulfillment is reached in at most $t$ attempts after the system stabilizes. % this sentence is weird todo
Note that this is particularly important in a partial-synchronous system since there are no guarantees on how long the system will remain stable. Thus, if the synchronous phases are too short and too many reconfiguration steps are required to reach a robust state the system could be stuck indefinitely.

\begin{definition}
\textbf{$t$-Bounded Conformity}: a recurringly robust evolving graph $\mathcal{G}$ exhibits \textit{$t$-bounded conformity} if a robust static graph appears in $\mathcal{G}$ at least once every $t$ consecutive static graphs. \label{def:boundedconformity}
\end{definition}

Note that, in a leader based system subject to $f$ faults, it is impossible to ensure fulfillment in less that $f+1$ attempts. Consider, for an instance a clique topology as found in \textit{PBFT}. Even though in the clique there are connections among all processes, the protocol will not be able to make any progress under a faulty leader, thus preventing fulfillment from being reached.
%Consider, for instance an evolving graph based on a star topology, where a leader process is placed in the center of the star (a communication pattern used for instance in \textit{HotStuff}). Clearly, if the process placed at the center is faulty it may prevent fulfillment from being reached.
This requires a view change to select a new leader and in the scope of this work, a reconfiguration of the communication graph by moving from static graph $G_k$ to static graph $G_{k+1}$. However, the new leader might also be faulty and, thus, in the worst case, considering $f$ consecutive faulty leaders, consensus may only be reached after $f+1$ reconfigurations. In a system where $f$ processes may be faulty, we say that an evolving graph offers optimal conformity if it satisfies $(f+1)$-bounded conformity.

Interestingly, for general topologies it may be hard, or even impossible to achieve optimal conformity. Consider for instance an evolving graph where all static graphs are binary trees. The number of possible binary trees is factorial with the number of processes and, from all these trees, only a small fraction is robust. An evolving graph that is constructed by a simple permutation among all possible configurations of the tree could require a factorial number of attempts. In fact, a fundamental challenge of using arbitrary topologies is to construct the evolving graph in a way that ensures optimal conformity.

\subsection{Cryptographic Principles}

However, while reconfiguration guarantees that eventually a sufficient number of signatures may be collected,  we assume the existence of sufficiently strong cryptographic primitives to fulfill the remaining properties. Thus, we must implement collections in a way that prevents Byzantine processes from tampering with values being propagated over the graph, and also prevents Byzantine processes from creating spurious values without being detected.

We implement this with the help of an abstract data type called a \textit{cryptographic collection}, a secure multi-set of tuples $(p_i, v_i)$. A process $p_i$ can create a new collection $c$ with a value $v_i$ by calling $c$=\textsc{new}($(p_i, v_i)$). Processes can also merge two collections using a \textsc{combine} primitive, 
$c_{12}$ = \textsc{combine}$(c_1, c_2)$, also denoted by $c_{12} = c_1 \oplus c_2$. Finally, a process can check if a collection $c$ includes at least a given threshold of $t$ distinct tuples with the same value $v$, by calling \textsc{has}$(c, v, t)$. Additionally, it is possible to check the total amount of input tuples that were contributed to $c$ by checking its cardinality $\vert c \vert$. Cryptographic collections have the following properties:

\begin{itemize}
    \item \emph{Commutativity:}   $c_1 \oplus c_2 = c_2 \oplus c_1$.
    \item \emph{Associativity:}   $c_1 \oplus (c_2 \oplus c_3)  = (c_1 \oplus c_2) \oplus c_3$.
    \item \emph{Idempotency:} $c_1 \oplus c_1 = c_1$.
    \item \emph{Integrity:} Let $c= c_1 \oplus \ldots c_i \ldots c_n$. If \textsc{has} ($c, v, t$) then at least $t$ distinct processes $p_i$ have executed $c_i$=\textsc{new}($(p_i, v)$).
\end{itemize}

Note that different cryptographic techniques can be used to implement these collections. The simplest implementation is to use regular public key cryptography to sign each value, and implement the collection as a set of individually signed values. The \textsc{new} primitive uses a regular signature scheme to produce a signed value and the \textsc{combine} primitive returns the union of the individually signed values included in the two input collections. The \textsc{has} primitive iterates over the collection, validates the signatures and counts the distinct tuples. A limitation of this implementation is that the size of the collection grows linearly with the number of processes, even when multiple processes input the same value. The entire collection of votes would have to be verified at all processes which hinders the scalability of the approach.

However, it is also possible to use more advanced techniques, to reduce the size of messages, in particular when the same value appears multiple times in a collection, something that is common in the execution of consensus protocols. Threshold signatures~\cite{threshold} and multisignatures\cite{multisig} are techniques that have been used in different consensus protocol for blockchains, such as HotStuff~\cite{hotstuff}, Motor~\cite{motor}, and Byzcoin~\cite{byzcoin}.

Threshold signatures, may be used to aggregate all signatures if a sufficient quorum is obtained at the root or center node allowing each process to verify the combined signature in $\mathcal{O}(1)$ steps which speeds up the process significantly. However, the root or center node still has to verify all signatures which still leads to a significant bottleneck.

\textit{Multisignatures} as used in \cite{byzcoin} avoid this problem. However, while they rely on \textit{schnorr signatures} which are highly efficient, they require an interactive protocol which requires three rounds of communication to build a single combined signatures which results in a significant latency trade-off.

We, therefore leverage aggregated \textit{bls signatures} as \cite{bls} which allow to aggregate the signature at each step in the tree. This way, the internal nodes may aggregate and verify the signatures they receive of their child nodes which distributes the verification and aggregation load over all internal nodes.
While \textit{bls signatures} have these interesting properties they are computationally much more expensive than traditional asymmetric signatures or \textit{schnorr signatures} which makes them only viable in larger scale systems.


==> older-versions/kauri-202012101447.tex <==
\section{Kauri}
\label{sec:thesystem}

We now introduce \thesystem.
The design of \thesystem is centered around three main objectives: 
%The contributions of this paper are centered on the communication patterns used to convey information from participants to the leader and from the leader to the participants, such that the 
i) reduced message complexity, ii) load balancing and iii) upon failures, reconfiguration in an optimal number of steps.
%up is reduced, load balancing  is achieved, and reconfiguration in an optimal number of steps can still be performed. 
Rather than proposing a new consensus protocol from scratch, we focus instead on the communication patterns and reconfiguration process necessary to achieve the objectives above.

To simplify our presentation, we frame our contributions within the scope of HotStuff, but our techniques are generic and can be applied to other leader-based consensus algorithms.
We also use the publicly available implementation of HotStuff as a baseline later in our evaluation (Section~\ref{sec:evaluation}).


With this in mind, we start by providing a brief description of HotStuff with the goal of identifying and extracting the communication primitives and patterns (Section~\ref{sec:overview}).
Next, we show how these patterns can be modified, without changing the original algorithm, to use different communication patterns with the aim of achieving the objectives above.

%\mm{to be completed}

\subsection{Overview}
\label{sec:overview}

\input{hotstuff}

Algorithm~\ref{algo:consensusalgo} shows the main algorithm of HotStuff
Broadly, it consists of three communication rounds, where each round has two generic steps:
i) the leader sends some information to all processes and, ii) processes reply back (i.e. vote) to the leader.
Initially, when bootstrapping the system, the leader creates a new block, appends it to its local copy of the blockchain and broadcasts this \textit{proposal} to all processes (lines~\ref{algo2:line:init}---\ref{algo2:line:init-end}).
Upon receiving a block proposal (lines~\ref{algo2:line:receiveblock}---\ref{algo2:line:receiveblock-end}), each process verifies if the block is valid (i.e. contains  valid transactions only), and checks if it extends the local blockchain. If these conditions hold, the process appends the block to its local blockchain and sends a \textit{prepare} to the leader.

In the second phase, the leader upon receiving a proposal vote (lines~\ref{algo2:line:receivepreparevote}---\ref{algo2:line:receivepreparevote-end}) verifies its validity and upon receiving a $2f+1$ votes broadcasts the result as a \textit{pre-commit}.
Upon receiving a \textit{pre-commit}(lines~\ref{algo2:line:receiveprecommit}---\ref{algo2:line:receiveprecommit-end}), the process verify its validity and reply to the leader with a \textit{commit} vote.
The leader waits once more for $2f+1$ \textit{commit} votes, locks the decision and broadcasts the result as a \textit{commit} (lines~\ref{algo2:line:receiveprecommitvote}---\ref{algo2:line:receiveprecommitvote-end}).
Upon receiving the \textit{commit}, the remaining processes also lock the block and send a final \textit{decide} to the leader (lines~\ref{algo2:line:receivecommit}---\ref{algo2:line:receivecommit-end}).

Finally, on the receival of the third quorum, the leader will finalize the block and disseminate the obtained quorum as the decision. After the processes receive the decision, they also finalize the block and propagate the locked quorum commit in a \textit{new-view} vote to the next leader (lines \ref{algo2:line:receivecommitvote} to \ref{algo2:line:receivedecide-end}).

The leader process receives the votes for the new round (lines \ref{algo2:line:receivenewviewvote} to \ref{algo2:line:receivenewviewvote-end}) where each votes contains the quorum signature of the last decision each process had locked in. The leader verifies the votes and adds the signatures to its view. After obtaining $2f+1$ votes it creates a new block upon the highest decision vote it obtained and propagates it to the remaining processes as a \textit{prepare} message starting the entire process over again.


The resulting topology and communication pattern of HotStuff are depicted in Figure~\ref{fig:examplestar} and Figure~\ref{fig:threephasehotstuf}, respectively, for a network of seven processes.

\begin{figure}[!t]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.4\textwidth]{figures/hotstuffstar.pdf}
  \caption{Star topology for seven processes}
  \label{fig:examplestar}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/hotstuffalgo.pdf}
  \caption{Communication pattern with a star topology for seven processes ($p_0$ --- $p_6$) and one client ($C$)}
  \label{fig:threephasehotstuf}
\end{subfigure}

\caption{Topology and communication pattern for HotStuff with seven processes.}
\label{fig:star}
\end{figure}

The large number of communication steps (three phases each with two communication rounds) necessary to produce a block can result in poor throughput and latency. To overcome this limitation, HotStuff leverages the fact that each block in the blockchain depends on its predecessor to produce three blocks per consensus instance, instead of one. 
This is achieved by creating a new block in each phase of the protocol and piggybacking the quorum signature of the previous round with the new block. 
In detail, processes voting on a block $b_i$, verify the quorum of the previous block and implicitly vote on the two previous blocks $b_{i-1}$ and $b_{i-2}$.
In this variant of the algorithm, called \textit{Chained-HotStuff}, a new block is produced in each phase of the protocol resulting in a significant improvement in throughput.

\input{chained_hotstuff}

Algorithm~\ref{algo:consensusalgo} shows an outline of \textit{Chained-HotStuff}.
Initially the leader bootstraps the system by producing a block and broadcasting it to all processes (lines~\ref{algo:line:init}---\ref{algo:line:init-end}).

When receiving a new block $b_i$, (lines~\ref{algo:line:receiveblock}---\ref{algo:line:receiveblock-end}), each process verifies: i) if the block is valid, ii) if it extends the last received block and iii) if it contains a valid quorum signature (QC) of the previous phase. If all those criteria are fulfilled, the block is appended to the blockchain, the block before the previous block ($b{i-2}$) is finalized and the vote (signature) is sent to the leader.
The leader, when receiving votes from the other processes (lines~\ref{algo:line:receivevote}---\ref{algo:line:receivevote-end}), verifies each vote and applies them to the current block. After collecting a quorum of votes ($2f+1$), a new block is created (including the created QC) and broadcast to all the processes, which restarts the algorithm.

Note that, if a block $b_i$ is aborted, for instance due to a failure, because of the chaining, the two previous blocks ($b_{i-1}$ and $b{i-2}$) also need to be aborted and the consensus restarted for block $b{i-2}$.

As discussed in Section~\ref{sec:relatedwork}, the leader needs to communicate directly with $N-1$ processes, and verify all the received inputs. Therefore, and as we show in the evaluation (Section~\ref{sec:evaluation}), the CPU and/or the bandwidth at the leader can easily become a bottleneck.\mm{confirm we show this}

The key insight of this work is that we can radically change these properties (and bottlenecks) by simply modifying the communication primitives (i.e \texttt{broadcast} and \texttt{send}) without further changes to the consensus algorithm itself.

Our goal is therefore to replace the star topology and communication pattern depicted in Figure~\ref{fig:star} with a tree based topology and communication pattern as depicted in Figure~\ref{fig:tree}.
Therefore, instead of having the leader broadcast information to, and receive information from all processes, this is relayed gradually from parent to child and vice-versa.

Note that, due to its nature a tree is more sensitive to faults as the failure of a single interior node may prevent consensus from terminating.
In the following sections, we discuss how \thesystem builds dissemination trees such that the correctness properties of the original consensus algorithm are preserved.

%This way we may re-utilize the consensus algorithm outlined in Algorithm~\ref{algo:consensusalgo} by only adjusting the implementation of the communication primitives.

%Our implementation uses exactly the same structure, based on three rounds of communication as HotStuff. However, in \thesystem we replace the start topology for a tree topology, as illustrated in Figures~\ref{fig:exampletree} and~\ref{fig:threephase}.
%Our consensus algorithm is an adjusted version of HotStuff but instead of working on a star we leverage a tree topology. We, therefore, also assume a three phase protocol where in each phase a quorum of signatures has to be collected.

\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.4\textwidth]{figures/exampletree.pdf}
	\caption{Tree topology for seven processes}
  \label{fig:exampletree}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/threephase.pdf}
	\caption{Communication pattern with a tree topology for seven processes ($p_0$ --- $p_6$) and one client ($C$)}
  \label{fig:threephase}
\end{subfigure}
\caption{Tree topology and communication pattern for seven processes.}
\label{fig:tree}
\end{figure}


%While this results in additional latency due to the additional communication steps it distributes the aggregation and verification overhead of the signatures over a set of processes to improve the scalability.


%Since we follow the same general structure as HotStuff, the safety properties of the algorithm apply directly to our approach\mm{this is too vague, we need a better discussion here, which can appear later in the paper}. 
%However, due to the nature of a tree topology, ensuring liveness imposes an additional set of requirements and properties.
%We define and discuss those requirements and properties in the next section.

%The respective tree that matches the protocol highlighted in Figure~\ref{fig:threephase} can be found in Figure~\ref{fig:exampletree}.
%With $P_0$ at the root, through the internal processes $P_i$ down to the leaf processes $L_i$.

%MM: this is fundamental to show, but I'm not sure this is the right place
%This way, safety is guaranteed as proven in \cite{hotstuff}. While most of the liveness proof also applies in this case, collecting signatures over a tree topology is inherently more complex than over a star. 
%This is the case, since even if the root is a correct process, faulty internal nodes may not relay all correct signatures.

\input{abstractions}






\input{reconfiguration}

\input{pipelining}

==> older-versions/pipelining-202012111500.tex <==
\section{Pipelining and Piggybacking}


\begin{figure}
     \centering
	\includegraphics[width=\columnwidth]{figures/hotstuff-pipeline.pdf}
	\caption{Pipelining in HotStuff}
  \label{fig:hotstuff-pipelining}
\end{figure}

\begin{figure}
     \centering
	\includegraphics[width=0.7\columnwidth]{figures/kauri-pipeline.pdf}
	\caption{Pipelining in \thesystem}
  \label{fig:kauri-pipelining}
\end{figure}



%The three phase protocol is displayed in Figure~\ref{fig:threephase}.
Considering the simple tree topology depicted in Figure~\ref{fig:exampletree}, the leader process $P_0$ collects three quorums, distributes them to the internal nodes $P_1, P_2, P_3$ which in turn relay them to the leaf processes $L_1$ to $L_3$ (dotted lines).

The additional communication steps compared to the star topology is displayed using the dotted line. 
Note, that this comes at an additional latency costs due to the relay from the internal processes to the leafs. However, the distribution of the computational and bandwidth load yields substantial benefits at scale.
As we will see later, in certain scenarios it is even possible for the tree to provide better latency than the star based topology (Section~\mm{XXX, make sure we show this}).


Due to the additional latency inherit in the tree structure which is also amplified by a geo-distributed deployment the performance of the system is significantly throttled while the nodes stay most of the time idle.

We've, therefore, developed a pipelining scheme which is similar to the asynchronous consensus scheme in \cite{ebawa} but adjusted to work in our particular use-case.
Thus, we've not only adjusted the approach such that each block extends the previous block, but also to properly function in a tree topology.

\setlength{\textfloatsep}{0pt}
\begin{algorithm}[h!]
\scriptsize
\centering
\caption{Piped Kauri Algorithm}
\label{algo:pipedkauri}
\begin{algorithmic}[1]
\State{blockchain $\gets b_0$}
\State{view $\gets v_0$}
\State{id $\gets 0$} \Comment{The id of this process}
\State{pendingblocks $\gets 0$}
\State{maxpendingblocks $\gets x$}

\Function{\textsc{init}} { }
\If{$view.leader(id)$}
\State{blockchain.createBlock()}
\State{\textbf{broadcast} blockchain.getTopBlock()}
\EndIf
\EndFunction

\Upon{\textsc{timer}} { } \label{algopiped:line:timer}
\If{$view.leader(id) \land$ pendingblocks $<$ maxpendingblocks }
\State{blockchain.createBlock()}
\State{\textbf{broadcast} blockchain.getTopBlock()}
\State{pendingblocks++}
\EndIf
\EndUpon \label{algopiped:line:timer-end}

\Upon{\textsc{receive} $b_i$}
\If{$b_i$.isValid() $\land b_i$.parent = blockchain.getTopBlock() $\land$ verify($b_i.qc$)}
\State{blockchain.append($b_i$)}
\State{blockchain.finalize($i - $maxpendingblocks$ * 2$)} \label{algopiped:line:finalize}
\State{\textbf{send} sign($b_i$) \textbf{to leader}}
\EndIf
\EndUpon

\Upon{\textsc{receive} $v_i$}
\If{verify($v_i$)}
\State{blockchain.getTopBlock().addSignature($v_i$)}
\If{$\vert$blockchain.getTopBlock().qc$\vert \geq 2f+1$ }
\State{blockchain.createBlock()}
\State{\textbf{broadcast} blockchain.getTopBlock()}
\EndIf
\EndIf
\EndUpon

\end{algorithmic}
\end{algorithm}
\setlength{\textfloatsep}{5pt}

We've outlined the pseudocode of our approach in Algorithm~\ref{algo:pipedkauri}.
The algorithm is very similar to Algorithm~\ref{algo:consensusalgo} with only a few adjustments. First, we've added an additional \textsc{timer} function that produces additional blocks and broadcasts them to the child processes in regular intervals up to a certain max limit (Lines ~\ref{algopiped:line:timer} to \ref{algopiped:line:timer-end}). Finally, we've also had to adjust the block approval process in line~\ref{algopiped:line:finalize} where instead of finalizing always the block before the last block, now the number of asynchronously produced blocks have to be considered.

\begin{figure}[!htb]
     \centering
	\includegraphics[width=0.5\textwidth]{figures/pipelining.pdf}
	\caption{Pipelining scheme}
  \label{fig:pipelining}
\end{figure}

This process is also visually outlined in Figure~\ref{fig:pipelining}.
Where for each additional depth level compared to the star, we produce one additional block (thus 1 additional block at depth 3 in this example). Thus, after $b_0$ reached the halfway point, we dispatch $b_1$ extending $b_0$. Then, after a quorum for $b_0$ is collected we disseminate $b_2$ including the quorum signature of $b_0$. Sequentially the same for $b_3$ with the quorum signature of $b_1$. After $b_2$ then reaches a quorum signature again, we disseminate $b_4$ which  contains the quorum signature of $b_2$ (the same for $b_5$ and $b_3$). Finally, after $b_4$ reaches a quorum signature, we completed the 3 phases of consensus for $b_0$ and may finalize it. Case any of the blocks fails, we will have to rollback to the last finalized blocks and start over.

The asynchronous block production is particularly useful for tree topologies and can only be applied in a very limited number of scenarios for star or clique topologies.

We show this through a small example. Assuming a block size of $100kb$, and 1000 processes, the process at the root of a star or each process in a clique already require 100mbit/s bandwidth to propagate a single block a single time. Thus, independent of the actual latency in the system, the overall block production speed is already limited to less than one block per second. Based on this, the system is unable to leverage spare computation power during the transmission latency since the system is already suffering a bandwidth bottleneck and is unable to increase its throughput in any way.

A tree, on the other hand, would require only a fraction of the bandwidth. depending on the fanout. The smallest possible tree, with two internal nodes, requires each internal node to consume only half of the bandwidth and could produce twice the number of blocks. Based on that, during the transmission time one block could be pipelined.

We later show in Section~\ref{sec:evaluation} how in practise this type of pipelining can only be leveraged by a tree topology and how we use it to outperform the star topology by several factors.


==> older-versions/pipelining-202012291453.tex <==
\section{Pipelining and Piggybacking}
\label{sec:pipelining}

As described earlier, HotStuff requires four rounds of communication for each instance of consensus. If HotStuff waited for each instance to terminate before starting the next one, the system throughput would suffer significantly. Therefore, HotStuff relies on a pipelining optimization, where the $i+1$ instance of consensus is started optimistically, before instance $i$ terminated.
As a result, at any given time, nodes in the system participate in multiple instances of consensus by batching multiple messages into a single one.
%can exchange messages of multiple instances of consensus. This is optimized by piggybacking messages from multiple instances in a single network packet.

By following the same structure of HotStuff, \thesystem is also amenable to the same optimization.
However, because \thesystem uses a tree to disseminate and aggregate messages, the latency to terminate a given round, and hence a consensus instance, is substantially larger than in HotStuff.

Therefore, without additional mechanisms, \thesystem would have substantial idle periods resulting in lower throughput than actually possible considering the available network and computational resources.
In this section, we discuss how HotStuff's mechanisms can be adapted to leverage the load-balancing properties of tree topologies and, not only mitigate the effects of the higher per round latency, but also improve the overall throughput by leveraging parallelism.

\subsection{Pipelining in HotStuff}

We start by providing an overview of HotStuff's pipelining using as an example the same seven node system introduced in Figure~\ref{fig:star}.
Figure~\ref{fig:hotstuff-pipelining} illustrates the execution of multiple rounds (each round is depicted in a different colour). 
Consider the first round depicted in the figure (in yellow) that starts with the leader sending the block to all other processes. The overall time required for this task depends on the size of the data being transmitted (for simplicity, let us assume it is dominated by the block size), the available bandwidth, and the total number of nodes. To conclude a round, the leader has to collect a quorum of signatures. These signatures start flowing towards the leader as soon as the first process receives the message from the leader and sends its reply back. Thus, in practice, the dissemination and the aggregation procedures are executed in parallel. 
Also, by the time the leader finishes transmitting the block to the last process, it might have already received $2f+1$ signatures (\textit{quorum received} arrow in the figure) and hence it is already processing them while the dissemination terminates. 
Thus, as soon as the dissemination of the first round finishes the leader might already be able to start the second round of consensus. In parallel, HotStuff optimistically starts a new instance of consensus by piggybacking the messages of the first round of the next consensus instance with the messages of the second round of the current instance.
Because HotStuff uses three rounds of communication, this process can be repeated another time, resulting in messages that carry information from up to three pipelined instances of consensus.
%n a message of HotStuff to Thus, by the end of the second round of the first instance of consensus, HotStuff starts a new instance. It now piggybacks the messages from the third round of the first instance with the messages from the second round of the second instance and the messages from the first round of the third instance. As a result, HotStuff messages always carry information from three pipelined instances of consensus.
In the design of HotStuff, the depth of the pipeline (i.e., the maximum number of consensus instances that run in parallel) is thus equal to the number of communication rounds. 

\begin{figure}
     \centering
	\includegraphics[width=\columnwidth]{figures/hotstuff-pipelining.pdf}
	\caption{Pipelining in HotStuff}
  \label{fig:hotstuff-pipelining}
\end{figure}

\subsection{Pipelining in \thesystem}

In \thesystem, we enhanced the pipeling technique to fully leverage the load balancing properties of the tree. We illustrate this in Figure~\ref{fig:kauri-pipelining}. As with HotStuff, the aggregation phase of a given round starts before the dissemination phase is complete and, therefore, there is potential for parallelism between the two phases of the same round. However, in \thesystem, and in contrast to HotStuff, the root completes its dissemination long before it has collected a quorum of replies of that round. This is the case, since dissemination requires multiple hops to complete, and second because the number of messages the leader has to send is much smaller than in HotStuff.

Like HotStuff, \thesystem leverages this by having the leader start a new instance of consensus shortly after the root finished disseminating the messages of a previous instance. 
The key difference is that \thesystem is able to start multiple consensus instances during the execution of a single round of consensus.
In the example of Figure~\ref{fig:kauri-pipelining}, the leader is able to start 3 new instances during the execution of the first round of a given consensus instance. 
Note that, in this example, 
%\thesystem is also able to piggyback messages from different instances. However,  in \thesystem, there is a wider distance between the instances that are piggybacked together. In the example depicted in Figure~\ref{fig:kauri-pipelining}, 
the messages from the second round of instance 1 are piggybacked with messages from the first round of instance 4, \emph{i.e.} a message carries information from consensus instances/rounds that are farther away in the pipeline.
This increase in the pipeline depth allows for a higher degree of parallelism, and hence throughput, as we discuss in the following sections.
%Like in HotStuff, \thesystem can combine, in the same  message of three different instances of consensus. However, the consensus instances that share the same packet are father apart in the pipeline. Also, the depth of the pipeline is longer in \thesystem; in the example above, 9 instances of consensus can be executed in parallel at each point in time.

\begin{figure}
     \centering
	\includegraphics[width=0.7\columnwidth]{figures/kauri-pipelining.pdf}
	\caption{Pipelining in \thesystem}
  \label{fig:kauri-pipelining}
\end{figure}

\subsection{Pipelining Depth}
\label{sec:pipelining-throughput}

We now discuss the factors that affect the depth of the \thesystem's pipeline. Roughly speaking, the depth of the pipeline is given by the number of consensus instances the root node, or leader, is able to start during a round times the number of rounds of the protocol (three in our case, the same HotStuff).

To simplify the presentation, lets assume that the size of the messages sent by the root is dominated by the block size. %even when control information from other instances is piggybacked in the packets. 
Given the block size $B$, the network bandwidth $b$, and the fanout $m$ the time the root takes to send each message is $\frac{B}{b}$, and the time to execute the dissemination phase is given by $\frac{mB}{b}$. We denominate this as \textit{Busy Time} $BT = \frac{mB}{b}$

Let $T_{last}$ be the instant where the root sends the last message in a round. The root has to wait at least $h * \textit{RTT}$ to receive the last response, where \textit{RTT} is the average roundtrip time in the network and $h$ is the depth of the dissemination tree. We denominate this as the \textit{Idle Time} $IT = h RTT$

Therefore, the number of instances the root can start is bound by  $\frac{IT}{BT}$. 
To illustrate this, Table~\ref{tab:examples} provides some examples of the impact of the height, fanout, block size, network bandwidth and RTT on the maximum number of parallel instances. The table first illustrates how additional pipelining doesn't yield any benefit on star topologies and also, how with increasing round trip time the idle time increases linearly and thus, the potential number of parallel instances also increases. It also shows that with a constant fanout, even with an increase of depth and scale, the pipelining may be used to compensate the performance loss as well as that a decrease in fanout may allow to speedup the system significantly. Finally, it shows the direct relation between the blocksize and the bandwidth consumption.

\begin{table}[t]
\centering
{\scriptsize
\caption{Maximum number of parallel consensus instances (pipelining depth) for varying weights, processes, block sizes, bandwidth and latency.}
\label{tab:examples}
\begin{tabular}{|p{0.3cm}p{0.7cm}p{0.4cm}p{0.8cm}p{0.9cm}p{0.4cm}p{0.4cm}p{0.4cm}p{1cm}|}
\hline
\textbf{N} & \textbf{Height} & \textbf{Fanout} & \textbf{BlockSize} & \textbf{Bandwidth} & \textbf{RTT} & \textbf{Busy Time} & \textbf{Idle Time} & \textbf{Parallel Instances} \\
\hline
401 & 2 (star) & 400 & 100kb & 100mb & 0,20 & 0,4 & 0,2 & 0,5 \\
421 & 3 & 20 & 100kb & 100mb & 0,20 & 0,02 & 0,4 & 20 \\
421 & 3 & 20 & 100kb & 100mb & 0,10 & 0,02 & 0,2 & 10 \\
8420 & 4 & 20 & 100kb & 100mb & 0,20 & 0,02 & 0,6 & 30 \\
399 & 4 & 7 & 100kb & 100mb & 0,20 & 0,007 & 0,6 & 85,7 \\
421 & 3 & 20 & 10kb & 100mb & 0,20 & 0,002 & 0,4 & 200 \\
421 & 3 & 20 & 100kb & 1gb & 0,20 & 0,002 & 0,4 & 200 \\
\hline
\end{tabular}
}
\end{table}

\subsection{Maximum Speedup}

In HotStuff, the leader needs to send $N-1$ messages before it can start a new instance. In \thesystem, the leader needs to send $m$ messages (where $m$ is the fanout of the tree) before it is ready to start a new instance. Therefore the maximum speedup that can be achieved by \thesystem is bound by $\frac{N-1}{m}$. For instance, in a system of $400$ nodes, organized in a tree with fanout $20$, the maximum speedup \thesystem can offer is $19.95$.

%Note that, the lower the fanout, the higher the speedup provided by \thesystem. However, as discussed in Section~\ref{sec:limitations}, increasing the number of internal nodes results in longer reconfiguration times.
%This exposes a tradeoff between speedup and reconfiguration time that should be taken into account when deploying \thesystem.
%Therefore, in the implementation we need to balance the speedup with the reconfiguration speed. 
%Recall that in deployments where \thesystem  must ensure Optimal Conformity, 
%In particular, when \thesystem is configured to be able to be reconfigured in optimal time, 
%the number of internal nodes is limited by $I =\frac{af+a}{f+1}$ (for a tree of depth 3, $m=I$). 
%Thus, in a scenario with  arbitrarily deep and perfectly balanced trees, $m^{h-1} = I$, and hence    the maximum speedup is bound by $\frac{N-1}{\root h-1 \of a}$.\mm{?}


==> older-versions/reconfiguration-202012111200.tex <==
\section{Reconfiguration}
\label{sec:reconfiguration}

\subsubsection{Recurringly Robust Evolving Graph}

Even if we start from a robust graph, due to faults, \thesystem may be required to perform one or more reconfigurations of the graph (or view changes). 
Every reconfiguration defines a new overlay network that will be used by the processes to communicate. 
We can model the sequence of overlay networks used by \thesystem as an evolving graph, i.e., a sequence of static graphs. To ensure that eventually a robust graph is used, the evolving graph must hold the following property:

\begin{definition} 
\textbf{Recurringly Robust Evolving Graph:} An evolving graph $\mathcal{G}$ is denoted to be \textit{recurringly robust} iff robust static graphs appear infinitely often in its sequence. \label{def:recurringlyrobust}
\end{definition}

\subsubsection{$t$-Bounded Conformity}

Note that even though a recurringly robust evolving graph is sufficient to ensure that a robust graph will be eventually used by processes to communicate, it is not very interesting in practice because the number of reconfigurations that are necessary before a robust graph is found are potentially unbound. Ideally, we would like the system to use a robust graph after at most $t$ reconfigurations. We call this property of an evolving graph \textit{$t$-bounded conformity}. 

\begin{definition}
\textbf{$t$-Bounded Conformity}: a recurringly robust evolving graph $\mathcal{G}$ exhibits \textit{$t$-bounded conformity} if a robust static graph appears in $\mathcal{G}$ at least once every $t$ consecutive static graphs.\label{def:boundedconformity}
\end{definition}

Note that, in the worst case, any leader-based protocol may require at least $f+1$ reconfigurations, because a faulty leader can always prevent consensus from being reached in which case it needs to be replaced. Interestingly, for general topologies it may be hard, or even impossible to achieve $t$-bounded conformity. Consider, for instance, an evolving graph where all static graphs are binary trees. The number of possible binary trees is factorial with the number of processes and, from all these trees, only a small fraction is robust - i.e. those where faulty processes are not interior nodes. A naive evolving graph that is constructed by a simple permutation among all possible configurations of the tree could require therefore a factorial number of reconfigurations to find a robust graph. 

Ideally, we want to have a bound number of reconfigurations such that they grow linearly either with the size of the system $N$ or the number of faults $f$.
This leads us to the notion of \emph{Linear Conformity} and \emph{Optimal Conformity}, respectively, as defined below.
%Therefore, in a system where $f$ processes may be faulty, we ideally want to build an evolving graph that observes 
%\emph{Optimal Conformity}.

\begin{definition}
\textbf{Linear Conformity}: a recurringly robust evolving graph $\mathcal{G}$ has Linear conformity iff, $\mathcal{G}$ observes $t$-bounded conformity where $t=\mathcal{O}(N)$.
\label{def:optimalconformity}
\end{definition}

\begin{definition}
\textbf{Optimal Conformity}: a recurringly robust evolving graph $\mathcal{G}$ has Optimal conformity iff $\mathcal{G}$ observes $t$-bounded conformity where $t=f+1$ with $f=\floor{\frac{N-1}{3}}$.
\label{def:optimalconformity}
\end{definition}


We now introduce the algorithm for building an evolving graph where each static graph is a tree. Note that this is significantly harder than using stars due to the much larger number of possible graphs. In fact, while in a star topology with $N$ processes there are $N$ distinct graphs, if we consider, for instance, binary trees, the number of possible graphs is given by the Catalan number $C_n = \frac{(2N)!}{((N + 1)!N!}$. Additionally, for each tree, there are $N!$ possible assignments from processes to nodes in the graph.

To make the problem tractable, we restrict ourselves to a balanced tree topology with a fixed fanout. Given a fixed topology, the remaining challenge is to assign the processes to nodes in the tree such that the resulting evolving robust graph ensures Optimal Conformity.

Note that, despite this simplification, the number of possible configurations is still factorial in the number of processes. 
In fact, from all the assignments of processes to nodes in the tree, only a small fraction is guaranteed to yield robust trees. This is because any tree that has a faulty internal node cannot be guaranteed to be robust\footnote{A tree with a faulty internal node might be robust if all its children are also faulty. However, we assume the more general case where some children of any faulty internal node might be correct.}.
More precisely, for $N$ nodes of which $I$ are internal nodes (including the root), there are ${N\choose I}$ different assignment possibilities.

However, due to the presence of $f=\floor{\frac{N-1}{3}}$ faulty processes, not all of these assignments are robust. \mm{if we lack space we can simplify this analysis}
Given $f$ faulty processes, there are $\frac{(N-f)!}{ (N - f - I)!}$ robust trees, i.e. those whose internal nodes are not faulty. 
Therefore, the probability $p_I$ to build a robust static graph is given by: 

%This, divided by the total number of graphs $\frac{N!}{(N-I)!}$ gives us the probability $p_I$ to build a robust static graph $G_k$ (Displayed in Equation~\ref{eq:pk1}).

\begin{equation}
\centering
\label{eq:pk1}
p_I = \frac{\frac{(N-f)!}{ (N - f - I)!}}{\frac{N!}{(N-I)!}}
\end{equation}

For a star topology where $I=1$, %solving this is trivial since $\frac{N!}{(N-1)!} = N$ and based on that, $\frac{(N-f)!}{ (N - f - 1)!}$ results in the probability 
$p_I = \frac{N - f}{N}$ thus the probability to construct a robust static graph $G_k$ by randomly shuffling the assignment of processes to nodes in the graph is constant for any size of $N$. Therefore, even when using a naive reconfiguration strategy, a robust configuration is guaranteed within optimal steps.

However, for tree topologies, where the number of internal nodes $I$ tends to increases with the total number of processes $N$, the probability $p_I$ to construct a robust graph is much lower.
Since $f$ depends on $N$ and is given by $f=\floor{\frac{N-1}{3}}$ we can rewrite Equation~\ref{eq:pk1} as:

\begin{equation}
\centering
\label{eq:pk2}
p_I = \frac{\frac{(N-\floor{\frac{N-1}{3}})!}{ (N-\floor{\frac{(N-1)}{3}} - I)!}}{\frac{N!}{(N-I)!}}
\end{equation}

Based on this, the main factor that determines the probability $p_I$ is the number of internal nodes $I$.
For example, considering $\lim\limits_{N\to\infty}p_I$ for $I=4$ the probability to build a robust graph, is  $\approx 20\%$ and for $I=10$ it is $\approx 1.7\%$. 
As the total number of internal nodes $I$ in the tree increases, the probability of finding a robust tree using a naive or randomized strategy becomes vanishingly small.
In fact, in the worst case, the required number of configurations is factorial to the number of internal nodes $I$.
This is the main reason why state of the art approaches that rely on trees degrade to a star or clique topology upon failures.
Next, we introduce our algorithm to overcome this problem.

\paragraph*{Build evolving graphs with Optimal Conformity}

Since in general we cannot distinguish among situations such as an internal node not forwarding the votes of its children, a faulty child processes that did not vote in the first place, or a process that is just slow due to asynchrony~\cite{flp}, upon an unsuccessful consensus, we have to suspect that all internal nodes are potentially faulty.
This observation, leads us to our key insight: if we split all processes into $f+1$ disjoint bins then at least one of those bins is guaranteed to have only correct nodes. 
By constructing a tree whose internal nodes are exclusively draw from this bin, we are guaranteed to obtain a robust tree.
%the only way to achieve Optimal Conformity is to split all processes into at least $f+1$ or more bins such that there must be at least one bin of solely correct processes to select internal nodes from. 
For this to work, we must have $\frac{N}{I} \geq f + 1$, i.e. there are sufficient processes to divide all processes into $f+1$ bins of size $I$.

%\setlength{\textfloatsep}{0pt}
\begin{algorithm}[!t]
\scriptsize
\centering
\caption{Construction of an Evolving Graph with Optimal Conformity}
\label{algo:robustGraph}
\begin{algorithmic}[1]

\Function{init}{$N,I,f$}
\label{algo:robustGraph:init}
%\State{$\mathcal{N} \gets B^0 \cup B^1 \cup \ldots \cup B^{\frac{N}{I}}$; s.t. $|B^i| \geq f+1 \land B^i \cap B^j = \emptyset$. }
\State{$\mathcal{N} \gets B^0 \cup B^1 \cup \ldots \cup B^{\frac{N}{I}}$; s.t. $|B^i| \geq f+1 \land B^i \cap B^j = \emptyset$. } \Comment{Build disjoint bins}
\label{algo:robustGraph:init:end}
\EndFunction

\Function{build}{$k$} 
\State{$i \gets k\;\textbf{mod}\;I$}\label{alg:e-tree:iteration}
\State{$\mathcal{G}^i \gets$ all possible trees whose internal nodes are drawn exclusively from bin $B^{i}$. }
\State{$T \gets$~pick any tree from $\mathcal{G}^i$}
\label{alg:e-tree:iteration:end}
\State{$ T \gets$~add as leaves of $T$ the processes that are not in $B^i$}
\State{$\textit{root}_k \gets T.\textsc{root}()$}
\State{$G_k^{in} \gets$ all edges of $T$ directed from the leaves to the root}
\State{$G_k^{out} \gets$ all edges of $T$ directed from the root to the leaves}
\State{\textbf{return}(root, $G_k^{out}$, $G_k^{in}$)}\label{alg:e-tree:return}
\EndFunction
\end{algorithmic}
\end{algorithm}

The algorithm for constructing a robust tree is show in Algorithm~\ref{algo:robustGraph}.
It receives as input the total number of processes, the number of internal nodes in the tree and the number of faulty processes, and divides them into $\frac{N}{I}$ disjoint bins (lines~\ref{algo:robustGraph:init}---\ref{algo:robustGraph:init:end}). 
Next, to build tree $\mathcal{G}_k$,
%and For each view $i$ we pick one of the $\frac{N}{I}$ bins (Line~\ref{alg:e-tree:iteration}) and construct a random tree where the internal nodes are exclusively drawn from this bin (Lines~\ref{alg:e-tree:iteration} to \ref{alg:e-tree:return}). 
%The algorithm is pretty straight forward. The tree is initiated with a set of processed $\mathcal{N}$ that are divided into a set of bins $B^i$. 
it picks bin $B^i$ following a round robin strategy and builds a random tree composed of nodes exclusively from $B^i$ (lines~\ref{alg:e-tree:iteration}---\ref{alg:e-tree:iteration:end}).
Finally, it adds the processes on the remaining bins as leaves in the tree, and creates the directed edges between the parent and children\mm{do we still need directed edges?}
%$B^i$ is picked and a random graph is constructed in which the processes in $B^i$ will serve as internal nodes and the remaining processes as leave nodes. We prove the correctness of this algorithm next.
Despite simple, Algorithm~\ref{algo:robustGraph} constructs trees that observe Optimal Conformity.
\begin{theorem}
\label{th:generictree}
\thesystem satisfies Optimal Conformity for any evolving Graph $\mathcal{G}$ iff $\frac{N}{I} \geq f + 1$.
\end{theorem}
\begin{proof}
We present all the proofs in Section~\ref{sec:proofs}.
\end{proof}

\paragraph*{Build evolving graphs with Linear Conformity}
\label{sec:linear}
While in an ideal scenario we want to have an evolving graph that observes Optimal Conformity this might not be possible in certain scenarios.
In fact, and as per Theorem~\ref{th:generictree}, it is not possible to achieve Optimal Conformity in a system where $\frac{N}{I} < f + 1$ holds.
%(as proven in Theorem~\ref{th:generictree}) 
However, in such scenarios it is still possible to construct an evolving graph that observes Linear Conformity as we sketch below.

%In the following we iteratively construct algorithms that achieve a robust configuration within linear steps. Since those algorithms are significantly more complex than the optimal algorithm outlined before, we iteratively expand the algorithm to improve the understanding of the inner workings.

%First, depict an algorithm that achieves very close to Optimal Conformity using clever combinatorics.

As a motivating example, consider a system with $N=7$ processes,  where $f=2$ can be faulty, and $I=3$ interior nodes deployed as a a balanced binary tree as depicted in Figure~\ref{fig:bintree}.
Note that under the constraint $\frac{N}{I} < f + 1$ it is not possible to evenly divide $N$ into $f+1$ bins.
In our example $7$ is not divisible by $3$ and hence we have to split the nodes into $f=2$ bins and we are left with $L=1$ leftover nodes (Figure~\ref{fig:bintreerotation}).
Therefore, and in general, we have two cases: a) either each of the $f$ bins contain exactly one faulty node and hence all leftover nodes $L$ are correct, or b) some bin contains only correct nodes. 
By leveraging this observation, we are able to devise a bin rotation strategy that builds an evolving graph that observes Linear Conformity.
The algorithm starts by constructing $f$ bins, and upon each iteration of the evolving graph a static tree $\mathcal{G}_k$ is generated whose interior nodes are draw from bin $B^i$ similarly to Algorithm~\ref{algo:robustGraph}. 
If after iterating over the $f$ bins no robust tree is found, we can safely assume that each bin contains exactly one fault node and thus all leftover nodes are correct.
Therefore, in the next 
%Because it is not possible to evenly divide the number of processes $N$ by the number of 
%If , then 
%When dividing the total number of processes $N$ by the number of internal nodes $I$ there is a possibility that the result is a fraction between $f$ and $f+1$. Thus, while it might not be possible to divide all processes into $f+1$ distinct bins, it is possible to divide all processes into $f$ distinct bins and have $L$ processes leftover that are not assigned to any bin.
%If, in the worst case, none of the $f$ bins results in a robust tree, we can safely assume that there is one faulty process in each bin and that none of the remaining processes in $L$ may be faulty.
iteration we replace the $I$ processes in one of the $f$ bins, step by step, with the leftover processes of $L$ until a robust tree is found, as depicted in Figure~\ref{fig:bintreerotation} (Steps $I$ to $IV$).
Since there are $I=3$ processes in the bin, in at most $3$ additional steps ($\frac{I}{L}$ steps in the general case), we have found a robust tree.
With this rotation strategy, we are able to construct a robust tree in $f + \frac{I}{L}$ steps in the worst case (since none of the $L$ leftover processes is faulty, with multiple leftover processes we can replace multiple processes in the bin at a time).

{
\begin{figure}[!t]
\begin{subfigure}[b]{.4\columnwidth}
  \centering
  	\includegraphics[width=0.3\linewidth]{figures/Tree.pdf}
  \caption{Balanced Binary Tree.}
  \label{fig:bintree}
\end{subfigure}
\begin{subfigure}[b]{.4\columnwidth}
  \centering
  \includegraphics[width=0.3\linewidth]{figures/bins.pdf}
	\caption{Bin rotation.}
  \label{fig:bintreerotation}
\end{subfigure}
\caption{Balanced binary tree with $N=7$, $I=3$ and $f=2$ and bin rotation strategy. Faulty nodes are shown in red.}
\end{figure}
}

%In Figure~\ref{fig:tree} we show an example of the outlined algorithm. 
%Assuming a balanced binary tree of depth $2$ resulting in a total of $N=7$ processes and $I=3$ internal nodes and, following $N=3f+1$ there are $f=2$ faulty nodes (highlighted red in the figure). Following $\frac{N}{I} < f+1$ we can't easily build $f+1$ distinct bins. 
%However, there are $\frac{N}{I} > f$ processes, resulting in $f$ distinct bins and $L=1$ leftover processes.

%Following this, as displayed in Figure~\ref{fig:rot}, after constructing trees using the $2$ bins of size $3$, in the next step we replace the members of one of the bins with the leftover process until a robust tree is found. 

\begin{theorem}
\thesystem satisfies Linear Conformity for any evolving Graph $\mathcal{G}$ if $\frac{N}{I} > f$.
\label{theo:lc1}
\end{theorem}

Theorem~\ref{theo:lc1} can be further relaxed to $\frac{N}{I} + L \geq f + 1$ provided that $\frac{N}{I} \geq L$ holds.
%can be even further relaxed to $\frac{N}{I} + L \geq f + 1$ as long as 
%This is quite similar to the previous approach, however, it is able to leverage multiple leftover replicas $L$ in a neat fashion.
In fact, and following the same rationale as above, $\frac{N}{I} + L \geq f + 1$ implies that: a) there is either one faulty process per bin and all but one of the leftover processes are faulty or, b) there are two faulty processes in all but one of the bins and all $L$ processes are correct.

Therefore, it is possible to rotate each leftover process $L_i$ within each bin $B^i$ and ensure that we end up with a bin composed exclusively of correct processes which in turn can be used to build a robust tree as per Algorithm~\ref{algo:robustGraph}.

%we by combining one of the leftover processes in $L$ each with a distinct bin and at least one of these bins may have at most one faulty process we're trivially able to achieve a robust tree.
To illustrate this strategy, consider the example in Figure~\ref{fig:rotGeneric} for $N=10$ processes, of which $f=3$ are faulty, and a total of $I=4$ internal nodes. 
Following $\frac{N}{I}$ we have $\frac{N}{I}=2$ bins of  size of $I=4$ and $L=2$ leftover processes. 
Since there is at least one faulty process per bin, after two reconfigurations (once per bin), it is not possible to build a robust tree (Figure~\ref{fig:rot3}). 
Thus, we must combine each leftover processes with the respective bin. 
First we combine the first processes with the first bin (steps $II$ to $V$). 
If this was unsuccessful, we know that either there must be two faulty processes in this bin or the leftover node is faulty. However, this implies that according to $f$, there is at most one faulty process in the remaining bin and the remaining leftover process must also be correct. Therefore, in the final step, after rotating the second leftover process over the second bin we are guaranteed to have a bin composed exclusively of correct processes (step $VI$).

\begin{figure}[!t]
   \begin{subfigure}{0.48\textwidth}
     \centering
	\includegraphics[width=0.4\textwidth]{figures/Tree3.pdf}
	\caption{Generic Tree}
  \label{fig:tree3}
   \end{subfigure}
   \begin{subfigure}{0.48\textwidth}
     \centering
	\includegraphics[width=0.4\textwidth]{figures/rot3.pdf}
	\caption{Bin rotation}
	\label{fig:rot3}
   \end{subfigure}
   \caption{Generic tree with $N=10$, $I=4$ and $f=3$ and bin rotation strategy. Faulty nodes are shown in red.}
   	\label{fig:rotGeneric}
\end{figure}

This rotation strategy is always executed in linear steps since each leftover process in $L$ is at most rotated over one bin. Thus, the complexity is the same as rotating one process over all processes in $N$, resulting in $\frac{N}{I} + N$.

\begin{theorem}
\thesystem satisfies linear Conformity for any evolving Graph $\mathcal{G}$ if $\frac{N}{I} + L \geq f+1$ as long as $\frac{N}{I} \geq L$.
\label{th:linear}
\end{theorem}


Theorem~\ref{th:linear} leads to an interesting insight.
In the particular case where $\frac{N}{I} = L$, and considering that $N=3f+1$ we have that 
%$\frac{N}{I} + \frac{N}{I} \geq f+1$
%$\frac{N}{I} + L \geq f+1$ with the condition of $\frac{N}{I} \geq L$ at the corner case of $\frac{N}{I} = L$ can be simplified to . If we insert also $N=3f+1$ this results in 
$\frac{3f+1}{I} + \frac{3f+1}{I} \geq f+1$ which, solving to $I$ results in 
%can be simplified to
%$\frac{6f+2}{I} \geq f+1$
$I=\frac{6f+2}{f+1}$.
Interestingly, this relation between $I$ and $f$ highlights a key limitation: given that $\lim\limits_{f\to\infty}{I}=6$,
%stays strictly below $6$. Therefore, by using this approach it 
it is not possible to build a robust tree in linear steps with more than 5 internal nodes (including the root). 

%Further, we observe that in all of our linear approaches $f$ stays strictly below $\frac{N}{I} * 2$. We prove next that this is indeed the minimum condition for any linear reconfiguration strategy.
This has important  implications in the types of deployments one can do in practice, which we capture in Theorem~\ref{th:nolinear} and further discuss in the following section.

\begin{theorem}
\label{th:nolinear}
It is impossible to design linear reconfiguration strategies for $f > \frac{N}{I} * 2$.
\end{theorem}



\subsection{Practical Reconfigurations}
We now discuss the practical implications of the above theorems.
Following Theorem~\ref{th:generictree}, we need $\frac{N}{I} \geq f + 1$ to achieve Optimal Conformity.
For a typical system with $N=3f+1$ processes, this can be rewritten to $I=\frac{3f+1}{f+1}$ which results in $\lim\limits_{f\to\infty}{I} = 3$.
This implies that, to achieve Optimal Conformity, and respecting $N=3f+1$, one is restricted to have at most two interior nodes, including the root.

While this might look dismally at first, it is possible to overcome this limitation in practice by adjusting the ratio of $N=3f+1$.
For instance by setting $N=3f+3$ one can have one more internal node and by setting $N=af+1$ where $ 3 \le a < I$ we can can tolerate $a-1$ internal nodes. 
More generically, by setting $N=af+a$ one can have $a$ internal nodes and still achieve Optimal Conformity.

%Based on $\frac{3f+1}{f+1} = I$ we have to relax our failure assumption to find a robust tree with an increasing number of internal Nodes. There are two ways to increase the number of internal nodes while continuing to guarantee optimal conformity. First, by adding additional processes to the second part of the equation. While maintaining near optimal fault tolerance, the number of internal nodes can be increased by one ($N = 3f+3$ instead of $N = 3f+1$).

%Second, from $\frac{3f+1}{f+1} = I$, we can reason that in order to be able to achieve optimal conformity with more than $2$ internal nodes we can also relax the first part of the equation. Thus, with decreasing restrictions ($3f+1, 4f+1, 5f+1, If+1$) it is possible to build topologies with more internal nodes ($2,3,4,...,I-1$).

%Both approaches can also be combined to maximize the number of internal nodes per tolerated fault ($N = 3f+3, 4f+4, 5f+5, If+I$ for $I = 3,4,5,...N$).

If the higher total number of nodes $N$ necessary to tolerate $f$ faults is deemed too costly, it is  possible to have a configuration with a smaller $N$ that still ensures Linear Conformity, provided there are at most $5$ internal nodes (as per Theorem~\ref{th:linear}).
%Sacrificing optimal conformity while maintaining linear reconfiguration steps allows to increase the maximum number of internal nodes to $5$ which is the upper limit for linear approaches (as we've also proven in Section~\ref{sec:thesystem}).
This highlights an important practical dilemma:
either reconfiguration time is more important and therefore one selects Optimal Conformity which requires a larger ratio between $N$ and $f$, or it is more important to have a better balance between $N$ and $f$ and hence one must pay the larger reconfiguration times of Linear Conformity.

%tthe optimallity of the reconfiguration strategy has to be sacrificed in order to balance the load over more processes, and/or the total number of faults in the function of $N$ may be relaxed (to $If+I$) in order to be able to reconfigure a tree with greater numbers of internal nodes.


\begin{table}[]
\centering
%{\footnotesize

\begin{tabular}{|c|ccccc|} 
\hline
\textbf{Conformity} & $I \leq \frac{N}{200}$ & $I \leq \frac{N}{100}$ & $I \leq \frac{N}{20}$ & $I \leq \frac{N}{10}$ & $I \leq \frac{N}{4}$ \\ \hline
\textbf{Optimal} & $f=199$ & $f=99$ & $f=19$ & $f=9$ & $f=3$ \\
\textbf{Linear} & $f=398$ & $f=198$ & $f=38$ & $f=18$ & $f=6$ \\ \hline
\end{tabular}
%}
\caption{Relation between Internal Nodes ($I$) and Failures ($f$) for Optimal and Linear Conformity scenarios with $N \ge 1000$ processes and $f \leq \frac{N}{3} + 1$}
\label{tab_scaling}
\end{table}

Table~\ref{tab_scaling} shows the relation among these factors for a large number of processes $N \ge 1000$.
For instance, to ensure Linear Conformity and have at most 10 interior nodes ($I \ge \frac{N}{100}$) it is possible to tolerate at most $198$ faulty processes.

%of the total percentage of internal nodes to the maximum number of failures for each of the approaches\footnote{The displayed numbers describe the limits for larger numbers of processes ($N \geq 1000$) while $f \leq \frac{N}{3} + 1$}. Therefore, depending on the graph it is possible to find a robust graph even in the presence of a high number of simultaneous faults in optimal or linear steps. In the worst case this will result in $2 * f+1$ or $2 * N$ steps.


Thus, instead of falling back to a star or clique we use a hybrid approach. We first attempt to reconfigure the tree under a reduced failure assumption.
Then, if, after a certain number of steps no robust configuration was found, we may still fall back to a tree with a reduced numbers of internal nodes instead of falling back to a star.

This is viable, since in practise the probability of a large number of simultaneous failures is highly unlikely. Additionally, even in the case of a large number of simultaneous failures, by distributing processes over bins randomly, there is still a high probability to find a robust configuration within linear or even optimal steps.


Approaches like \textit{Motor} or \textit{Omniledger} that also offer reconfiguration strategies for trees require in the worst case $\frac{N}{fanout} * f+1$ which is significantly higher than the approach we propose in this paper. Additionally, these approaches do not offer an actual recovery strategy and stay for a potentially unbound time in the performance deprived state.

Thus, even with reduced failure assumptions as above, the random reconfiguration strategy of the two approaches will, where our approach will find an optimal configuration in $f+1$ reconfiguration steps, remain $60-70\%$ of the time in a performance deprived state and for the setting where we find an optimal reconfiguration in $N$ steps, even close to $90\%$ of the time\footnote{Probability that at least one of the $f$ faulty nodes is chosen by random as an internal node}.


%\setlength{\textfloatsep}{0pt}
%\begin{algorithm}[!t]
%\scriptsize
%\centering
%\caption{Implementation of the Networking Primitives}
%\label{algo:scheduleTree}
%%\begin{algorithmic}[1]
%\State{$k \gets 0$} \Comment{Current instance number}
%\State{$\mathcal{G} \gets build(k)$}
%\State{$c \gets \emptyset$}

%\Function{\textsc{broadcast}} {$b$}
%\State{\textbf{send} to $\mathcal{G}.getChildren(this)$}
%\EndFunction
%\Function{\textsc{send-to-leader}} {$v$}
%\State{\textbf{send} to $\mathcal{G}.getParent(this)$}
%\EndFunction

%\Upon{\textsc{receive} ($b$)} {}
%\State{\textbf{send} to $\mathcal{G}.getChildren(this)$}
%\EndUpon \label{algo:line:receiveblock-end}

%\Upon{\textsc{receive} ($v$)} {}
%\If{$verify(v)$}
%\State{\textsc{combine}($c$, $v$)}
%\If{\textsc{has}($c$, $v$, $\vert \mathcal{G}.getChildren(this) %\vert$)}
%\State{\textbf{send} to $\mathcal{G}.getParent(this)$}
%\EndIf
%\EndIf
%\EndUpon \label{algo:line:receiveblock-end}

%\end{algorithmic}
%\end{algorithm}
%\setlength{\textfloatsep}{5pt}


\mm{TODO: we still miss the alg. that puts eveything together: tree constuction, communication and crypto primitives}


==> older-versions/reconfiguration-202012221220.tex <==
\section{Reconfiguration}
\label{sec:reconfiguration}

%\subsubsection{Recurringly Robust Evolving Graph}

We now discuss \thesystem's reconfiguration strategy.
A reconfiguration is required when, due to faults or during an instability period, the  current configuration is not robust. 
%Note that even if we start from a robust graph, due to faults, \thesystem will be eventually required to perform one or more reconfigurations of the graph (or view changes). 
Every reconfiguration corresponds to a new graph which is materialized by a new overlay network that processes use to communicate. 
Naturally, not all the graphs are robust and several reconfigurations might be required before a robust graph is found.
We model the sequence of graphs  as an evolving graph, i.e., a sequence of static graphs. To ensure that eventually a robust graph is used, the evolving graph must hold the following property:

\begin{definition} 
\textbf{Recurringly Robust Evolving Graph:} An evolving graph $\mathcal{G}$ is said to be \textit{recurringly robust} iff robust static graphs appear infinitely often in its sequence. \label{def:recurringlyrobust}
\end{definition}

%\subsubsection{$t$-Bounded Conformity}

Note that even though a recurringly robust evolving graph is sufficient to ensure that a robust graph will be eventually used by processes to communicate, it is not very interesting in practice because the number of reconfigurations that are necessary before a robust graph is found are potentially unbound. Ideally, we would like the system to find a robust graph after at most a target number $t$ of  reconfigurations. We call this property of an evolving graph \textit{$t$-bounded conformity}. 

\begin{definition}
\textbf{$t$-Bounded Conformity}: a recurringly robust evolving graph $\mathcal{G}$ exhibits \textit{$t$-bounded conformity} if a robust static graph appears in $\mathcal{G}$ at least once every $t$ consecutive static graphs.\label{def:boundedconformity}
\end{definition}

Note that, in the worst case, any leader-based protocol may require at least $f+1$ reconfigurations, because a faulty leader may always prevent consensus from being reached in which case it needs to be replaced. Interestingly, for general topologies it may be hard, or even impossible to achieve $t$-bounded conformity. Consider, for instance, an evolving graph where all static graphs are binary trees. The number of possible binary trees is factorial with the number of processes and, from all these trees, only a small fraction is robust - i.e. those where faulty processes are not interior nodes. A naive evolving graph that is constructed by a simple permutation among all possible configurations of the tree could require therefore a factorial number of reconfigurations to find a robust graph. 

Ideally, we want to have a bound number of reconfigurations such that they grow linearly either with the size of the system $N$ or the number of faults $f$.
This leads us to the notion of \emph{Optimal Conformity}, as defined below.
%
\begin{definition}
\textbf{Optimal Conformity}: a recurringly robust evolving graph $\mathcal{G}$ has Optimal conformity iff $\mathcal{G}$ observes $t=f+1$-bounded conformity.% with $f=\floor{\frac{N-1}{3}}$.
\label{def:optimalconformity}
\end{definition}

We now introduce the algorithm for building an evolving graph where each static graph is a tree. Note that this is significantly harder than using stars due to the much larger number of possible graphs. In fact, while in a star topology with $N$ processes there are $N$ distinct graphs, if we consider, for instance, binary trees, the number of possible graphs is given by the Catalan number $C_n = \frac{(2N)!}{((N + 1)!N!}$. Additionally, for each tree, there are $N!$ possible assignments from processes to nodes in the graph.

To make the problem tractable, we restrict ourselves to a balanced tree topology with a fixed fanout. Given a fixed topology, the remaining challenge is to assign the processes to nodes in the tree such that the resulting evolving robust graph ensures Optimal Conformity.

Note that, despite this simplification, the number of possible configurations is still factorial in the number of processes. 
In fact, from all the assignments of processes to nodes in the tree, only a small fraction is guaranteed to yield robust trees. This is because any tree that has a faulty internal node cannot be guaranteed to be robust\footnote{A tree with a faulty internal node might be robust if all its children are also faulty. However, we assume the more general case where some children of any faulty internal node might be correct.}.
More precisely, for $N$ nodes of which $I$ are internal nodes (including the root), there are ${N\choose I}$ different assignment possibilities.

However, due to the presence of $f=\floor{\frac{N-1}{3}}$ faulty processes, not all of these assignments are robust. \mm{if we lack space we can simplify this analysis}
Given $f$ faulty processes, there are $\frac{(N-f)!}{ (N - f - I)!}$ robust trees, i.e. those whose internal nodes are not faulty. 
Therefore, the probability $p_I$ to build a robust static graph is given by: 

%This, divided by the total number of graphs $\frac{N!}{(N-I)!}$ gives us the probability $p_I$ to build a robust static graph $G_k$ (Displayed in Equation~\ref{eq:pk1}).

\begin{equation}
\centering
\label{eq:pk1}
p_I = \frac{\frac{(N-f)!}{ (N-f-I)!}}{\frac{N!}{(N-I)!}}
\end{equation}

For a star topology where $I=1$, %solving this is trivial since $\frac{N!}{(N-1)!} = N$ and based on that, $\frac{(N-f)!}{ (N-f-1)!}$ results in the probability 
$p_I = \frac{N-f}{N}$ thus the probability to construct a robust static graph $G_k$ by randomly shuffling the assignment of processes to nodes in the graph is constant for any size of $N$. Therefore, even when using a naive reconfiguration strategy, a robust configuration is guaranteed within optimal steps.

However, for tree topologies, where the number of internal nodes $I$ tends to increase with the total number of processes $N$, the probability $p_I$ to construct a robust graph is much lower. Since $f$ depends on $N$ and is given by $f=\floor{\frac{N-1}{3}}$ we can rewrite Equation~\ref{eq:pk1} as:

\begin{equation}
\centering
\label{eq:pk2}
p_I = \frac{\frac{(N-\floor{\frac{N-1}{3}})!}{ (N-\floor{\frac{(N-1)}{3}} - I)!}}{\frac{N!}{(N-I)!}}
\end{equation}

Based on this, the main factor that determines the probability $p_I$ is the number of internal nodes $I$.
For example, considering $\lim\limits_{N\to\infty}p_I$ for $I=4$ the probability to build a robust graph, is  $\approx 20\%$ and for $I=10$ it is $\approx 1.7\%$. 
As the total number of internal nodes $I$ in the tree increases, the probability of finding a robust tree using a naive or randomized strategy becomes vanishingly small.
In fact, in the worst case, the required number of configurations is factorial to the number of internal nodes $I$.
This is the main reason why state of the art approaches that rely on trees degrade to a star or clique topology upon failures.
Next, we introduce our algorithm to overcome this problem.

\paragraph*{Build evolving graphs with Optimal Conformity}

Since in general we cannot distinguish among situations such as an internal node not forwarding the votes of its children, a faulty child processes that did not vote in the first place, or a process that is just slow due to asynchrony~\cite{flp}, upon an unsuccessful consensus, we have to suspect that all internal nodes are potentially faulty.
This observation, leads us to our key insight: if we split all processes into $f+1$ disjoint bins then at least one of those bins is guaranteed to have solely correct nodes. 
By constructing a tree whose internal nodes are exclusively drawn from this bin, we are guaranteed to obtain a robust tree.
%the only way to achieve Optimal Conformity is to split all processes into at least $f+1$ or more bins such that there must be at least one bin of solely correct processes to select internal nodes from. 
For this to work, we must have $\frac{N}{I} \geq f + 1$, i.e. there are sufficient processes to divide all processes into $f+1$ bins of size $I$.

%\setlength{\textfloatsep}{0pt}
\begin{algorithm}[!t]
\scriptsize
\centering
\caption{Construction of an Evolving Graph with Optimal Conformity}
\label{algo:robustGraph}
\begin{algorithmic}[1]

\Function{init}{$N,I,f$}
\label{algo:robustGraph:init}
%\State{$\mathcal{N} \gets B^0 \cup B^1 \cup \ldots \cup B^{\frac{N}{I}}$; s.t. $|B^i| \geq f+1 \land B^i \cap B^j = \emptyset$. }
\State{$\mathcal{N} \gets B^0 \cup B^1 \cup \ldots \cup B^{\frac{N}{I}}$; s.t. $|B^i| \geq f+1 \land B^i \cap B^j = \emptyset$. } \Comment{Build disjoint bins}
\label{algo:robustGraph:init:end}
\EndFunction

\Function{build}{$k$} 
\State{$i \gets k\;\textbf{mod}\;I$}\label{alg:e-tree:iteration}
\State{$\mathcal{G}^i \gets$ all possible trees whose internal nodes are drawn exclusively from bin $B^{i}$. }
\State{$T \gets$~pick any tree from $\mathcal{G}^i$}
\label{alg:e-tree:iteration:end}
\State{$ T \gets$~add as leaves of $T$ the processes that are not in $B^i$}
\State{$\textit{root}_k \gets T.\textsc{root}()$}
\State{$G_k^{in} \gets$ all edges of $T$ directed from the leaves to the root}
\State{$G_k^{out} \gets$ all edges of $T$ directed from the root to the leaves}
\State{\textbf{return}(root, $G_k^{out}$, $G_k^{in}$)}\label{alg:e-tree:return}
\EndFunction
\end{algorithmic}
\end{algorithm}

The algorithm for constructing a robust tree is shown in Algorithm~\ref{algo:robustGraph}.
It receives as input the total number of processes, the number of internal nodes in the tree and the number of faulty processes, and divides them into $\frac{N}{I}$ disjoint bins (lines~\ref{algo:robustGraph:init}---\ref{algo:robustGraph:init:end}). 
Next, to build tree $\mathcal{G}_k$,
%and For each view $i$ we pick one of the $\frac{N}{I}$ bins (Line~\ref{alg:e-tree:iteration}) and construct a random tree where the internal nodes are exclusively drawn from this bin (Lines~\ref{alg:e-tree:iteration} to \ref{alg:e-tree:return}). 
%The algorithm is pretty straight forward. The tree is initiated with a set of processed $\mathcal{N}$ that are divided into a set of bins $B^i$. 
it picks bin $B^i$ following a round robin strategy and builds a random tree composed of internal nodes exclusively from $B^i$ (lines~\ref{alg:e-tree:iteration}---\ref{alg:e-tree:iteration:end}).
Finally, it adds the processes of the remaining bins as leaves in the tree, and creates the directed edges between the parent and child nodes\mm{do we still need directed edges?}
%$B^i$ is picked and a random graph is constructed in which the processes in $B^i$ will serve as internal nodes and the remaining processes as leave nodes. We prove the correctness of this algorithm next.
Despite simple, Algorithm~\ref{algo:robustGraph} constructs trees that observes Optimal Conformity.

\begin{theorem}
\label{th:generictree}
\thesystem satisfies Optimal Conformity for any evolving Graph $\mathcal{G}$ iff $\frac{N}{I} \geq f + 1$
\end{theorem}

\begin{proof}
We prove this in two steps.
First we prove that if $\frac{N}{I} \geq f + 1$ Optimal Conformity can be achieved, then, in the second step we proof that Optimal Conformity in a generic tree can only be achieved if and only if $\frac{N}{I} \geq f + 1$.

We divide all processes into bins where in each iteration $k$ the processes of a distinct bin are selected as internal nodes.

Simply, to divide all processes into bins of size $I$ we divide the total number of processes $N$ by the number of internal nodes $I$ resulting in $\frac{N}{I}$ bins.
Therefore, as long as $\frac{N}{I} \geq f + 1$ there are $f+1$ or more bins and, trivially there must be one bin without any faulty nodes resulting in a correct configuration after at most $f+1$ attempts. Thus, Optimal Conformity is observed.

In the second step, we prove that, in the worst case, it is not possible to achieve Optimal Conformity deterministically unless this condition is met. We proof this by contradiction. Thus, we assume there has to be a tree topology that is able to achieve Optimal Conformity where $\frac{N}{I} < f$.

As discussed, a set of correct internal nodes is required to guarantee a robust tree. However, since we can not make any assumptions about which of the internal nodes lead to past failures we have to replace the entire set of internal nodes in each step. Thus, to achieve optimal conformity we require a sequence of $f+1$ sets of internal nodes such that, in the worst case, the $f+1^{th}$ set consists solely of correct processes.

Considering $\frac{N}{I} < f$, it is not possible to divide all processes in $f+1$ bins of the size of $I$ with distinct processes in each bin. To create $f+1$ bins, at least one node must appear in multiple bins. However, this could be a faulty node, resulting in a faulty node in each of the $f+1$ bins. Similarly, if the processes are divided into less or equal to $f$ bins, each bin also may contain at least one faulty node.

Based on that, there are only two possibilities. Either the tree structure has to tolerate faulty internal nodes or it has to be possible to detect a faulty internal node to exchange it. Otherwise more than $f+1$ steps are necessary to find a robust configuration.
The first is not possible since there are no redundant communication paths in a tree and
the latter is also not possible since under partial synchrony it is impossible to distinguish a faulty node from a node that is slow or in an asynchronous phase\cite{flp}.
This leads to a contradiction.
Therefore, more than $f+1$ steps are necessary to find a robust configuration for $\frac{N}{I} < f$ leading to a contradiction since at most $f+1$ steps are allowed to observe Optimal Conformity.
\end{proof}

\paragraph*{Limitations}
\label{sec:limitations}

We now discuss the practical implications of the above theorems.
Following Theorem~\ref{th:generictree}, we need $\frac{N}{I} \geq f + 1$ to achieve Optimal Conformity.
For a typical system with $N=3f+1$ processes, this can be rewritten to $I=\frac{3f+1}{f+1}$ which results in $\lim\limits_{f\to\infty}{I} = 3$.
This implies that, to achieve Optimal Conformity, and respecting $N=3f+1$, one is restricted to have at most two internal nodes, including the root.

While this might look dismally at first, it is possible to overcome this limitation in practice by adjusting the ratio of $N=3f+1$.
For instance by setting $N=3f+3$ one can have one more internal node and by setting $N=af+1$ where $ 3 \le a < I$ we can can tolerate $a-1$ internal nodes. 
More generically, by setting $N=af+a$ one can have $a$ internal nodes and still achieve Optimal Conformity (i.e: for $1\%$ internal nodes we might tolerate up to $99$ faults).
This leads to an important dilemma. Either the load balancing properties are more important and the failure assumptions have to be reduced, or it is more important to tolerate large quantities of simultaneous failures and a tree with less internal nodes has to be used.

There is also the possibility of a hybrid approach where initially the tree is reconfigured with a reduced failure assumption and after $f+1$ steps without achieving a robust configuration the system falls back to a tree with reduced load balancing.
This is viable, since in practise the probability of a large number of simultaneous failures is highly unlikely. Additionally, even in the case of a large number of simultaneous failures, by distributing processes over bins randomly, there is still a high probability to find a robust configuration within optimal steps.

%Approaches like \textit{Motor} or \textit{Omniledger} that also offer reconfiguration strategies for trees require in the worst case $\frac{N}{fanout} * f+1$ which is significantly higher than the approach we propose in this paper. Additionally, these approaches do not offer an actual recovery strategy and stay for a potentially unbound time in the performance deprived state.

%Thus, even with reduced failure assumptions as above, the random reconfiguration strategy of the two approaches will, where our approach will find an optimal configuration in $f+1$ reconfiguration steps, remain $60-70\%$ of the time in a performance deprived state and for the setting where we find an optimal reconfiguration in $N$ steps, even close to $90\%$ of the time\footnote{Probability that at least one of the $f$ faulty nodes is chosen by random as an internal node}.

\paragraph*{Integration with HotStuff}

Applying the tree reconfiguration to HotStuff is then trivial. Natively, in HotStuff, after no consensus is achieved, each process compiles a \textit{new-view} message, includes the last successful quorum in it and selects a new leader to which it sends the message. The proponent leader awaits $2f+1$ \textit{new-view} messages and then publishes a new block to bootstrap the protocol again including the quorum of \textit{new-view} votes serving as a proof of the election.
Similarly, on timeout, with \thesystem, each process invokes the \textsc{build} function of Algorithm~\ref{algo:robustGraph} to construct a new tree and sends the same \textit{new-view} message to the new root of the tree. The root then also gathers $2f+1$ signatures before re-initiating the protocol.

==> older-versions/relatedwork-202011121500.tex <==
%% Related Work (Discuss PBFT, then HotStuff (discuss how the implementation uses libsec because bls would perform very badly since they are slow if the center has to verify and aggregate all themselves (bottleneck)), and then the other tree structures, table with: 
% Reconfiguration Strategy,
% Throughput comparison
% Arbitrary Trees
%

\section{Related Work}
\label{sec:relatedwork}

\begin{table}[]
\centering
{\footnotesize
\caption{Comparison of existing Algorithms}
\label{tab_comparison}
\begin{tabular}{|l|c|c|c|c|}
\hline\hline
 & \textbf{Reconf.}  & \textbf{Arbitrary}  & \textbf{Throughput}  &  \textbf{Recovery}\\ 
\textbf{Algorithm} &  \textbf{Strategy} & \textbf{Trees} & \textbf{Comparison}  & \textbf{Strategy} \\ \hline
 \multicolumn{4}{c}{\textit{previous work}}\\\hline
 Steward\cite{pbft} & X  & X  & \checkmark & X\\ 
 Byzcoin\cite{byzcoin} & X  & \checkmark & X & X\\ 
 Motor\cite{motor} & \checkmark  & X & X & X\\
 Omniledger\cite{omniledger} & \checkmark  & X & X & X\\\hline
 \multicolumn{4}{c}{\textit{Proposed algorithm}}\\\hline
 This paper & \checkmark  & \checkmark & \checkmark & \checkmark \\
\hline\hline
\end{tabular}
}
\end{table}

The problem of Byzantine agreement was originally discussed in the context of synchronous systems\cite{byzGens}, where it has been solved using a recursive algorithm that has factorial message complexity. Most Byzantine consensus protocols used today have been inspired by the \textit{PBFT} algorithm\cite{pbft}, which guarantees safety in a completely asynchronous setting but requires synchronous phases to guarantee progress. While \textit{PBFT} relies on an \textit{all-to-all} communication scheme, and hence a clique topology that results in a quadratic message complexity, for a small numbers of processes it provides excellent throughput and latency. For this reason, numerous algorithms extended \textit{PBFT} maintaining the same communication scheme and topology but slightly altering the protocol~\cite{ebawa, Archer}.

Other approaches explore different trade-offs by relying on  alternative topologies. \textit{HotStuff} is a recent proposal that uses a communication pattern based on a star-topology~\cite{hotstuff}. The algorithm used by \textit{HotStuff} requires three rounds of communication where, in each round, the replica at the center of the star collects partial signatures from all replicas and then distributes threshold signatures.  Therefore, \textit{HotStuff} has linear communication complexity.  Note that, even if the authors point out the usage of threshold signatures\cite{hotstuff}, the publicly available prototype at the time of this writting uses \textit{libsecp256k1}\cite{libsec} (a highly efficient\footnote{Although LibSec is highly efficient,  multiple attack vectors have been identified against it\cite{savecurves}.} elliptical curve algorithm that is also used in Bitcoin).

While this allows \textit{HotStuff} to perform very well, it limits the scalability and puts a lot of strain on network resources. Nonetheless, if for higher scales threshold or bls signatures were used, this would result in a bottleneck at the process in the center of the star. This is the case, since verifying bls signatures takes over 30 times longer than the used signature scheme (libsecp256k1) as we show in Section~\ref{sec:evaluation}.

A way to distribute the load to avoid this bottleneck while keeping the message complexity low is to organize the participants in hierarchical groups.

One of the first works that leverages hierarchies is \textit{Steward}~\cite{steward} that relies on a two level hierarchy where there are different failure assumptions for the specific levels of the hierarchy and each group uses threshold signatures to represent their decision in the overall consensus algorithm. While this performs very well in medium sized groups it doesn't scale very well since the protocol that is used within each group and on the level between the groups still requires a quadratic number of messages to be exchanged. While other solutions like \textit{Fireplug}~\cite{fireplug} avoid a quadratic message complexity in the local groups, they are still limited to a two level hierarchy and require quadratic messages on the inter-group level.

This may be mitigated by organizing the processes in hierarchical dissemination/aggregation trees. One prominent example of this is \textit{Byzcoin} that gathers signatures in a hierarchical structure using collective signing in two \textit{PBFT}-alike phases. Collective signing works in a binary tree structure and allows the coordinator to efficiently gather quorums to impose its decision on the remaining replicas. This requires three interactive rounds up and down the binary tree to build one collective signature. However, if no consensus is achieved, the protocol falls back to an \textit{all-to-all} communication scheme.

\textit{Motor} builds upon the principles of \textit{Byzcoin}, but instead of falling back to a clique topology, it uses a scheduler that rotates the replicas in the subtrees until the coordinator is able to gather $N-f$ signatures. \textit{Motor} states that robust trees require exponential steps to be built, hence they only build a tree up to two levels deep, consisting out of $c$ groups. Thus, assuming a correct leader, in the worst case, $\frac{N}{c}$ reconfiguration steps are necessary to construct a robust tree. Based on that, assuming in the worst case $f+1$ sequential faulty leaders, $(f + 1) * \frac{N}{c}$ steps are necessary.
Also, different to \textit{Byzcoin}, \textit{Motor} leverages bls signatures to avoid the costly interactive protocol.

\textit{Omniledger}~\cite{omniledger} also tries to avoid falling back to an \textit{all-to-all} communication scheme by also fixing the structure to a two-level hierarchy. Processes are assigned to different positions in the tree at random. If a process within a group does not respond with a sufficient quantity of votes the protocol leader queries additional processes in that group until a sufficient quantity of votes is obtained resulting in a similar "fallback-strategy" as \textit{Motor}.

A comparison of different approaches can be found in Table~\ref{tab_comparison}. While \textit{Steward} is the only solution that offers a throughput comparison with other high throughput byzantine fault tolerant consensus protocols it lacks a strategy to build and automatically reconfigure the structure in the presence of failures. Similarly, it also does not support any more complex structures of arbitrary depth.

\textit{Byzcoin} does support more complex trees, however, it only offers a performance comparison with \textit{Bitcoin} and falls back to a clique in the presence of failures.

While both \textit{Motor} and \textit{Omniledger} avoid falling back to a clique by attempting to query other processes in the lower levels of the hierarchy, however, that forces them to restrict the topology to a two level hierarchy. Additionally, neither of them offers a performance comparison with a high throughput protocol.

Lastly and most importantly, none of the proposed algorithms discuss or offer recovery strategies. After a failure of an internal node in the tree, the approaches potentially stay for an unbound period of time in the deprived state.

==> older-versions/relatedwork-202011240900.tex <==
%% Related Work (Discuss PBFT, then HotStuff (discuss how the implementation uses libsec because bls would perform very badly since they are slow if the center has to verify and aggregate all themselves (bottleneck)), and then the other tree structures, table with: 
% Reconfiguration Strategy,
% Throughput comparison
% Arbitrary Trees
%

\section{Related Work}
\label{sec:relatedwork}

The problem of Byzantine agreement was originally discussed in the context of synchronous systems\cite{byzGens} where it has been solved using a recursive algorithm with factorial message complexity. Most Byzantine consensus protocols used today have been inspired by the PBFT algorithm\cite{pbft} which guarantees safety in a completely asynchronous setting but requires synchronous phases to guarantee progress. PBFT organizes processes in a clique resulting in an \textit{all-to-all} communication scheme with quadratic message complexity. 
For a small numbers of processes, PBFT can offer excellent throughput and latency, but due to the quadratic message cost it does not scale to a large system. Although there are have been many proposals to extend and improve several aspects of PBFT (for instance, \cite{ebawa, Archer, bftsmart, spinning}) most preserve the same communication pattern.

The recent interest in permissioned blockchains, where consensus plays a crucial role, and the need to scale such systems to thousands of processes~\cite{sbft,libradocs}, fueled the research on alternative algorithms, with better scalability and load balancing properties.

HotStufforganizes processes in a star-topology~\cite{hotstuff} in order to reduce message complexity. 
It uses three communication rounds where, in each round, the replica at the center of the star plays the role of the leader and collects and distributes votes to and from all other replicas. The protocol has linear message complexity but creates a bottleneck at the leader, that needs to communicate with all the other processes and also needs to verify the signatures of every received message.

At the time of this writing, the publicly available implementation of HotStuff uses \textit{libsecp256k1}\cite{libsec}, a highly efficient elliptical curve algorithm also used in Bitcoin but against which several attack vectors have been found\cite{savecurves}.
Note that this requires HotStuff to relay all signatures votes to all other processes. 
Alternatively, and to reduce network load, it is possible to use threshold signatures at the expense of a significant increase in the load of the leader. For instance, the BLS threshold signatures are 30 times slower to verify than the signatures used in libsecp256k1 (see Section~\ref{sec:evaluation}). 

Systems such as Steward\cite{steward} and Fireplug\cite{fireplug} are able to distribute the load while keeping a low message complexity by organizing the processes in hierarchical groups. However, these systems still rely on an all-to-all communication pattern in the multicast group that stands at the root of the hierarchy and, therefore, to ensure scalability, make restrictive assumptions regarding the number and distribution of faults.

Another alternative is to organize processes in a tree topology which is used for dissemination and aggregation purposes. Byzcoin\cite{byzcoin} organizes processes in a binary tree where signatures (votes) are aggregated as they climb the tree from leaf nodes to the root, and the root uses the same tree to disseminate the results of the aggregation. While this design results in sublinear message complexity and has good load balancing properties, the failure of a single interior node can prevent progress. Byzcoin overcomes this difficulty by falling back to clique topology (which has quadratic message complexity) when faults are detected.

Motor\cite{motor} and Omniledger~\cite{omniledger} build upon the principles of Byzcoin, but instead of falling back immediately to a clique topology, they use a scheduler that rotates the replicas in the subtrees until the leader is able to gather $N-f$ signatures. If the process at the root of the tree is unable to collect sufficient signatures, they query leaf processes directly, which in turn will attempt to collect votes from their neighboring processes, until a quorum is obtained. Thus, in the worst case, assuming a fanout of $c$, after $\frac{N}{c}$ steps the tree will have collapsed to a star topology. Further, in the presence of a faulty leader a total of $(f + 1) * \frac{N}{c}$ might be necessary until liveness is reestablished.
For this to work, the tree must be limited to the depth of two, Motor justifies this by stating that finding a robust tree requires an exponential number of steps.

Strikingly, neither Motor or Omniledger propose a mechanism to move the system y back to the tree topology, after it has fallback to the degraded topology. Thus, as soon a fault occurs, these systems lose their desirable communication properties permanently. In a large scale system, where failure are the norm rather than the exception~\cite{failuresarecommon}, this implies that those systems are more likely to run in a degraded state than in the optimal one.

Table~\ref{tab_comparison} summarizes the properties of the systems described above.

\begin{table}[t]
\centering
{\scriptsize
\caption{Comparison of existing Algorithms}
\label{tab_comparison}
\begin{tabular}{|l|c|c|c|c|}
\hline
 & \textbf{Distributes the} & \textbf{Distributes the}    &  \textbf{Reconfigures in} & \textbf{Supports}\\ 
 & \textbf{processing} & \textbf{bandwidth}   &  \textbf{$t+1$} & \textbf{pipelining} \\ 
 & \textbf{load} & \textbf{consumption}   &  \textbf{steps} &  \\ 
\hline
%\textbf{Algorithm} &  \textbf{Balancing} & \textbf{Bottleneck} & \textbf{Bottleneck}  & \textbf{Conformity} \\ \hline
 %\multicolumn{4}{c}{\textit{previous work}}\\\hline
  HotStuff (BLS) \cite{hotstuff} & $\bullet$  & \checkmark &  \checkmark & \checkmark  \\ 
  HotStuff (LibSec) \cite{hotstuff} & $\bullet$  & $\bullet$   & \checkmark & \checkmark \\ 

 Steward\cite{steward} & $\bullet$  & $\bullet$   & $\bullet$ & $\bullet$ \\ 
 Byzcoin\cite{byzcoin} & \checkmark   & \checkmark & $\bullet$  & $\bullet$ \\ 
 Motor\cite{motor} & \checkmark  & \checkmark  & $\bullet$  & $\bullet$ \\
 Omniledger\cite{omniledger} & \checkmark  & \checkmark  & $\bullet$  & $\bullet$ \\\hline
 %\multicolumn{4}{c}{\textit{Proposed algorithm}}\\\hline
 \thesystem (this paper) & \checkmark  & \checkmark & \checkmark & \checkmark \\
\hline
\end{tabular}
}
\end{table}



In this paper we propose \thesystem, a system aimed at overcoming these limitations. \thesystem implements a reconfiguration strategy that is able to produce a robust tree in optimal (i.e. $f+1$) reconfiguration steps. We name this property as Optimal Conformity and formally defined it in Section~\ref{sec:thesystem}.

Table~\ref{tab_comparison} summarizes the properties of each system.

Overall, all of the state-of-the- art approaches have limitations in one or more aspects of Processing (load balancing among processes), bandwidth (message complexity and size of messages), latency (number of communication steps) and Optimal Conformity (Section~\ref{sec:thesystem}).

All of the approaches we've presented above, suffer bottlenecks on some degree which hinder the scalability of the approaches. In some approaches, like in HotStuff, a subset of processes (\textit{i.e.} the center node) has to process all signatures of all participating processes. Thus, with an increasing number of participants, eventually this subset of processes will turn itself a bottleneck and hinder the scalability.

Similarly, if a process has to send a large quantity of signatures to a large group of processes, eventually the system will run into bandwidth limitations also resulting into a bottleneck. This way, those approaches suffer scalability issues on the level of the bandwidth.

Finally, tree based approaches come with a trade-off where the throughput suffers depending on the depth of the tree and the average network latency between the nodes. A tree of depth tree (similar to Motor and Omniledger suffers twice the latency related cost compared to Hotstuff. Arbitrarily deep trees like Byzcoin suffer $(depth - 1)$ times the latency related cost compared to HotStuff. In Section~\ref{sec:evaluation} we show the impact of this additional cost on the throughput of the approach.

Another significant problem of approaches that leverage tree structures is, that not only a faulty leader results in a reconfiguration, but also a faulty internal node requires recovery steps to guarantee the collection of a quorum. To the best of our knowledge, none of the existing approaches offer an algorithm that achieves optimal conformity ($f+1$ steps) without falling back to a more simple structure (star or clique).
Additionally, none of these proposed algorithms discuss or offer recovery strategies. After falling back to a star or clique, the algorithms stay for an unbound period of time in this deprived state

==> older-versions/relatedwork-202012220830.tex <==
%% Related Work (Discuss PBFT, then HotStuff (discuss how the implementation uses libsec because bls would perform very badly since they are slow if the center has to verify and aggregate all themselves (bottleneck)), and then the other tree structures, table with: 
% Reconfiguration Strategy,
% Throughput comparison
% Arbitrary Trees
%

\section{Related Work}
\label{sec:relatedwork}

The problem of Byzantine agreement was originally discussed in the context of synchronous systems\cite{byzGens} where it has been solved using a recursive algorithm with factorial message complexity. Most Byzantine consensus protocols used today have been inspired by the PBFT algorithm\cite{pbft} which guarantees safety in a completely asynchronous setting but requires synchronous phases to guarantee progress. PBFT organizes processes in a clique resulting in an \textit{all-to-all} communication scheme with quadratic message complexity. For a small numbers of processes, PBFT can offer excellent throughput and latency, however, due to the quadratic message cost it does not scale to large system sizes. Although there have been many proposals to extend and improve several aspects of PBFT (for instance, \cite{ebawa, Archer, bftsmart, spinning}) most preserve the same communication pattern.

The recent interest in permissioned blockchains, where consensus plays a crucial role, and the need to scale such systems to thousands of processes\cite{sbft,libradocs}, fueled the research on alternative algorithms, with better scalability and load balancing properties.

HotStuff organizes processes in a star-topology in order to reduce message complexity\cite{hotstuff}. It uses three communication rounds where, in each round, the replica at the center of the star plays the role of the leader and collects and distributes votes to and from all other replicas. The protocol has linear message complexity but creates a bottleneck at the leader, that needs to communicate with all processes and also has to verify the signatures of $2f+1$ processes each round. 
At the time of writing, the publicly available implementation of HotStuff uses \textit{libsecp256k1}\cite{libsec}, a highly efficient elliptical curve algorithm also used in Bitcoin but against which several attack vectors have been found\cite{savecurves}. Note, this requires HotStuff to relay all signatures to all processes. Alternatively, and to reduce network load, it is possible to use threshold signatures at the expense of a significant increase in the load of the leader. For instance, \textit{bls signatures} are 30 times slower to verify than the signatures used in \textit{libsecp256k1} (see Section~\ref{sec:evaluation}). 

Another interesting feature of HotStuff is that it implements an optimization strategy known as \textit{pipelining}, that allows to overlap in time different rounds for different instances of consensus. Since consensus requires multiple rounds of communication, for better throughput, HotStuff can optimistically start the consensus for the next block before the consensus for the current block is terminated, allowing up to three consensus instances to run in parallel.

Systems such as Steward\cite{steward} and Fireplug\cite{fireplug} are able to distribute the load while keeping a low message complexity by organizing the processes in hierarchical groups. However, these systems still rely on an all-to-all communication pattern in the multicast group positioned at the root of the hierarchy and, therefore, to ensure scalability, make restrictive assumptions regarding the distribution of faults.

Another alternative is to organize processes in a tree topology which is used for dissemination and aggregation purposes. Byzcoin\cite{byzcoin} organizes processes in a binary tree where signatures (votes) are aggregated as they are relayed up the tree from the leaf nodes to the root, and the inverse to disseminate the results of the aggregation. While this design results in linear message complexity and has good load balancing properties, the failure of a single internal node can prevent progress. Byzcoin overcomes this difficulty by falling back to a clique topology (which has quadratic message complexity) when faults are detected.

Motor\cite{motor} and Omniledger\cite{omniledger} build upon the principles of Byzcoin, but instead of falling back immediately to a clique topology, they use a scheduler that rotates the replicas in the subtrees until the leader is able to gather $N-f$ signatures. If the process at the root of the tree is unable to collect sufficient signatures, they query leaf processes directly, which in turn will attempt to collect votes from their neighboring processes, until a quorum is obtained. Thus, in the worst case, assuming a fan-out of $c$, after $\frac{N}{c}$ steps the tree will have collapsed to a star topology. Further, in the presence of a faulty leader a total of $(f + 1) * \frac{N}{c}$ steps might be necessary until liveness is reestablished.
For this to work, the tree must be limited to the depth of two, Motor justifies this by stating that otherwise finding a robust tree requires an exponential number of steps.

Strikingly, neither Motor nor Omniledger propose mechanisms to move the system back to the tree topology, after the fallback to the degraded topology. Thus, in the presence of faulty processes, these systems lose their desirable communication properties permanently. In a large scale system, where failures are the norm rather than the exception\cite{failuresarecommon}, this implies that those systems are more likely to run in a degraded state than in the optimal one. 

Another disadvantage of using a multi-level tree to disseminate/ aggregate information in consensus is that it increases the number of communication steps per round of communication and, therefore, increases the latency. If consecutive consensus instances are executed in serial order, this increase in latency has also a negative impact on the throughput of the system. Such effect can be mitigated using and extending the pipelining techniques, such as the ones adopted by HotStuff.

Table~\ref{tab_comparison} summarizes the properties of the systems described above. Byzcoin, Motor, and Omniledger are able to distribute the processing load, because signatures are aggregated on their path to the leader, such that the leader does not need to verify all signatures. For the same reason, these systems are able to distribute bandwidth consumption among the root and the internal nodes of the distribution/aggregation tree, such that there is not a single process that needs to communicate with every other process. Unfortunately, neither of them are able to converge to a configuration that ensures the termination in an optimal number of steps. Also, none of these systems implements pipelining, which is key to mitigate the impact of the extra-latency on the system throughput.


\begin{table}[t]
\centering
{\scriptsize
\caption{Comparison of existing Algorithms}
\label{tab_comparison}
\begin{tabular}{|l|c|c|c|c|}
\hline
 & \textbf{Balances} & \textbf{Balances}    &  \textbf{$t+1$} & \textbf{Supports} \\ 
 
 & \textbf{processing} & \textbf{bandwidth}   &  \textbf{Reconfig.} & \textbf{Pipelining}\\  
 
 & \textbf{load} & \textbf{consumption}   &  \textbf{steps} &  \\ 
\hline
%\textbf{Algorithm} &  \textbf{Balancing} & \textbf{Bottleneck} & \textbf{Bottleneck}  & \textbf{Conformity} \\ \hline
 %\multicolumn{4}{c}{\textit{previous work}}\\\hline
 HotStuff (BLS)  & $\bullet$  & \checkmark &  \checkmark & \checkmark  \\ 
 HotStuff (LibSec)  & $\bullet$  & $\bullet$   & \checkmark & \checkmark \\ 
 Steward/ Fireplug & $\bullet$  & \checkmark  & $\bullet$ & $\bullet$ \\ 
 Byzcoin\ & \checkmark   & \checkmark & $\bullet$  & $\bullet$ \\ 
 Motor & \checkmark  & \checkmark  & $\bullet$  & $\bullet$ \\
 Omniledger & \checkmark  & \checkmark  & $\bullet$  & $\bullet$ \\\hline
 \thesystem (this paper) & \checkmark  & \checkmark & \checkmark & \checkmark \\
\hline
\end{tabular}
}
\end{table}

In this paper we propose \thesystem, a system aimed at overcoming the scalability limitations found in previous works. \thesystem owns the advantages of Byzcoin, Motor, and Omniledger, but without their disadvantages. Like these systems, \thesystem organizes the communication pattern on top of a tree to distribute both the processing load and the bandwidth utilization. Still, \thesystem implements a reconfiguration strategy that is able to produce a robust tree in optimal (i.e. $f+1$) reconfiguration steps. We name this property Optimal Conformity and formally defined it in Section~\ref{sec:trees}. Also, \thesystem leverages pipelining to hide the effects of the extra latency introduced by the tree. Instead of proposing our own Consensus Algorithm, \thesystem can be plugged into any hierarchical consensus algorithm to replace the communication scheme which results in increased throughput and improved load balancing.

==> older-versions/systemmodel-202011241413.tex <==
\section{System Model}
\label{sec:systemmodel}

The system is composed of a set of $N$ server processes $\{p_1, p_2, .. p_N\}$ and a set of client processes $\{c_1, c_2, .. c_m\}$. Client and server processes are connected through reliable communication channels (constructed by adding mechanisms for message retransmission as well as detecting and suppressing duplicates~\cite{cachinbook}). We also assume the existence of a \textit{Public-Key-Infrastructure} that is used by the replicas for authentication and signing. 

We assume the Byzantine fault model, where faulty processes may produce and return arbitrary values, delay or omit messages, and collude with each other, but do not possess sufficient computational power to compromise cryptographic primitives. Of the total set of $N$ processes, at most $f \leq \frac{N-1}{3}$  can be faulty. Furthermore, to circumvent the impossibility of consensus\cite{flp}, we assume a partially synchronous system.  Like other consensus protocols for this setting, \thesystem always ensures safety but can only ensure progress during synchronous periods~\cite{partial}.

The system can run multiple instances of consensus; typically, a different instances of consensus is executed 



We restrict ourselves to leader-based consensus algorithms, i.e., we assume that for each consensus instance there is one and only one process that performs the role of leader. We define each collection of one quorum as "one communication round" and the collection of sufficient quorums to produce a block as "one instance of consensus".
Furthermore, processes are organized in a logical tree and the leader process is placed at the root of that tree. The tree is used to propagate information from the remaining processes to the leader and from the leader to them. 

The collection of votes starts at the leaf processes which send their votes to their parents. 
Inner processes wait for inputs from their children, aggregate this information, and forward the aggregate to their parents. This process is repeated at each level of the three until the (aggregated) information reaches the root. When propagating information, the root sends data to its children, which in turn relay this information to their children, and so forth. Naturally, if the root or an inner node is faulty, this may prevent aggregation or data dissemination to terminate. Therefore, different consensus instances will use different trees.

To perform aggregation, we leverage the BLS non interactive cryptographic aggregation scheme that allows each inner node to aggregate the votes from its children into a single (aggregated) vote~\cite{bls}. 
The complexity of verifying an aggregated vote is $\mathcal{O}(1)$, thus the burden imposed on each inner node (including the root) is $\mathcal{O}(c)$, where $c$ is the fanout of the tree. 
%For this purpose we use the  BLS scheme presented in. 
Note that classical asymmetric signatures require $\mathcal{O}(N)$ verifications at every process and threshold signature schemes require $\mathcal{O}(N)$ at the root and $\mathcal{O}(1)$ at all the other processes\cite{bls}. 
Finally, we also assume that server processes may not change their keys during the execution of the protocol and require a sufficiently lengthy approval process to re-enter the system to avoid rogue key attacks~\cite{roguekey}.

% The rogue key attack one is important because all the well performing aggregated bls schemes do not work that well for completely open systems. Else we'd need an interactive one that needs several rounds up and down the tree. But in a permissioned system this is a valid assumption we can make.


==> older-versions/systemmodel-202012220850.tex <==
\section{System Model}
\label{sec:systemmodel}

The system is composed of a set of $N$ server processes $\{p_1, p_2, .. p_N\}$ and a set of client processes $\{c_1, c_2, .. c_m\}$. Client and server processes are connected through perfect point-to-point channels (constructed by adding mechanisms for message re-transmission as well as detecting and suppressing duplicates~\cite{cachinbook}). We also assume the existence of a \textit{Public-Key-Infrastructure} that is used by the replicas for authentication and signing. 
Moreover, processes may not change their keys during the execution of the protocol and require a sufficiently lengthy approval process to re-enter the system to avoid rogue key attacks~\cite{roguekey}.

We assume the Byzantine fault model, where faulty processes may produce and return arbitrary values, delay or omit messages, and collude with each other, but do not possess sufficient computational power to compromise cryptographic primitives. Of the total set of $N$ processes, at most $f \leq \frac{N-1}{3}$ can be faulty. 

Furthermore, to circumvent the impossibility of consensus\cite{flp}, we assume the partial synchrony model of~\cite{partial}. In this model, there may be an unstable period, where messages exchanged between correct processes can be delayed. Thus, while the system remains unstable, it is impossible to distinguish a faulty process from a slow process. However, there is some known bound $\Delta$ on the worst-case network latency and an unknown Global Stabilization Time (GST), such that after GST, all messages exchanged between correct processes arrive within $\Delta$.

%\mm{text below is not about the model, it needs to go somewhewre else}
%The system can run multiple instances of consensus; typically, a different instance of consensus is executed for each block before appending it to the blockchain. Each instance of consensus requires multiple rounds of communication. Each round is executed in a given system \textit{configuration} (also known as \textit{view}), where processes are organized in a logical tree to aggregate and disseminate information. \thesystem uses a leader based consensus algorithm, thus, in every configuration, there is a process that is designated as the leader; this process sits at the root of the communication tree. Different rounds of the same consensus instance may use different configurations. In particular, if the leader or an internal node of the tree is faulty, it may be impossible to terminate a consensus instance with that configuration. Thus, in faulty runs, it may be unavoidable to execute rounds in different configurations. In fault-free runs, its is possible to run all rounds required to terminate an instance using the same configuration.

%To perform aggregation, we leverage the BLS non interactive cryptographic aggregation scheme that allows each inner node to aggregate the votes from its children into a single (aggregated) vote~\cite{bls}. The complexity of verifying an aggregated vote is $\mathcal{O}(1)$, thus the burden imposed on each inner node (including the root) is $\mathcal{O}(c)$, where $c$ is the fanout of the tree.  Note that classical asymmetric signatures require $\mathcal{O}(N)$ verifications at every process and threshold signature schemes require $\mathcal{O}(N)$ at the root and $\mathcal{O}(1)$ at all the other processes\cite{bls}. 
%Finally, we also assume that server processes may not change their keys during the execution of the protocol and require a sufficiently lengthy approval process to re-enter the system to avoid rogue key attacks~\cite{roguekey}.

% The rogue key attack one is important because all the well performing aggregated bls schemes do not work that well for completely open systems. Else we'd need an interactive one that needs several rounds up and down the tree. But in a permissioned system this is a valid assumption we can make.


==> older-versions/trees-202012220913.tex <==
\section{From a Star to a Tree Topology}
\label{sec:trees}

Instead of designing a completely new consensus algorithm from scratch, we developed \thesystem as an adaptation of an existing protocol, in our case, as an adaptation of HotStuff. The key idea is that we solely have to replace the dissemination and aggregation patterns used by HotStuff that are based on a star topology, by new patterns based on dissemination/aggregations trees.

\subsection{HotStuff Communication Pattern}

Due to space constraints, it is not possible to provide a detailed description of HotStuff. However, for self-containment, we provide a very brief high-level description of its operation. We give emphasis on the communication pattern used in HotStuff and discuss how this pattern may be abstracted, to allow us to replace it with our more scalable implementation. HotStuff reaches consensus in four communication rounds. Each round consists of two phases: i) a dissemination phase where the leader broadcasts some information to all processes; ii) an aggregation phase where the leader collects and aggregates information that it received from a quorum of replicas. All rounds follow the same exact pattern, but the information sent and received by the leader in each round differs:

\begin{enumerate}
\item \textit{First round:} In the dissemination phase, the leader broadcasts a block proposal to all processes. In the aggregation phase, the leader collects a quorum of $2f+1$ signatures of the block. The signatures convey that  the replicas have validated and accepted the block proposed by the leader. We call this first quorum the \textit{prepare} quorum.

\item \textit{Second round:} In the dissemination phase, the leader broadcasts the \textit{prepare} quorum, either as a collection of individual signatures or a single combined signature, when threshold or aggregated signatures are used. In the aggregation phase, the leader again collects a quorum of signatures, this time of the \textit{prepare} quorum which imply that the processes have validated all signatures included in the quorum. We call this second quorum the \textit{pre-commit} quorum. If the leader is able to collect a quorum, the value proposed by the leader is \textit{locked} and it will not be changed, even if the leader is suspected and a reconfiguration occurs.

\item \textit{Third round:} In the dissemination phase, the leader broadcasts the \textit{pre-commit}. In the aggregation phase, the leader collects a quorum of signatures of the \textit{pre-commit} quorum, which as before imply that processes have validated the quorum. If the leader is able to collect a quorum, which we call the  \textit{commit} quorum), the leader decides and terminate.

\item \textit{Forth round:} Finally, in the last round, the leader disseminates the result in a decision message to all processes, which verify the final quorum and then send the last locked in decision to the leader of the next round to restart the process.
\end{enumerate}

\begin{figure}[!t]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.4\textwidth]{figures/hotstuffstar.pdf}
  \caption{Star topology for seven processes}
  \label{fig:examplestar}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/hotstuffalgo.pdf}
  \caption{Communication pattern with a star topology for seven processes ($p_0$ --- $p_6$) and one client ($C$)}
  \label{fig:threephasehotstuf}
\end{subfigure}

\caption{Topology and communication pattern for HotStuff with seven processes.}
\label{fig:star}
\end{figure}

Figure~\ref{fig:star} illustrates the communication pattern of HotStuff in a system with 7 processes. We can abstract the communication pattern used in HotStuff using the following two primitives:

\begin{itemize}
\item \textsl{disseminate-to-followers(data)}. This primitive is invoked by the leader; it is used in the first phase of each round to send data to all other processes. 
\item \textsl{aggregate = aggregate-at-leader(input$_i$, input$_j$, $\ldots$)}. This primitive is invoked by every non-faulty process $i$ that has received \textsl{data} from the leader in the first phase. The input by node $i$ consist of a cryptographic signature of \textsl{data}. The primitive returns an aggregate of the input signatures to the leader, containing at least $2f+1$ input values. 
\end{itemize}

While HotStuff uses one particular implementation of the two primitives above, we can assume that other implementations are possible as long as they offer the same guarantees. To characterize the guarantees provided by the communication pattern of HotStuff, we first define the notion of a \textit{robust configuration}. We say that the primitives are executed in a robust configuration if the leader is correct and in a non-robust configuration if the leader is faulty. Using this notion, we can capture the properties of the \textsl{disseminate-to-followers} and \textsl{aggregate-at-leader} primitives:

\begin{definition} 
\textbf{Reliable Dissemination:} After the Global Stabilization Time, and in a robust configuration, all correct processes deliver the \textsl{data} sent by the leader.
\end{definition}

\begin{definition} 
\textbf{Fulfilment:} After the  Global  Stabilization Time, and in a robust configuration, the aggregate collected by the leader includes at least $2f+1$ signatures.
\end{definition}

If the configuration is not robust, the primitives offer no guarantees. In particular, some nodes may receive the same \textsl{data} from the leader and others may receive no data at all or different \textsl{data}. The aggregation arriving at the leader may include less than $2f+1$ valid signatures, even if the leader sends consistent and valid data to all other nodes.
Note that, before the Global Stabilization Time is reached, it may be impossible to distinguish a robust from a non-robust configuration.

\subsection{Using Trees to Implement HotStuff}

We now discuss how to implement the \textsl{disseminate-to-followers} and \textsl{aggregate-at-leader} primitives using tree topologies, while preserving the same properties. As noted before, the idea is to organize the nodes in a tree hierarchy with the leader at the root. The primitive \textsl{disseminate-to-followers} is implemented by having the root send data to its children, that in turn forward this data to their own children, and so forth. The primitive \textsl{aggregate-at-leader} is implemented by having the leaf nodes send their signatures to their parent. The parent aggregates the signatures of its child processes with its own and sends the aggregate to their own parent. This process is repeated until the final aggregate is computed at the root of the tree. This process is illustrated in Figure~\ref{fig:tree}.

\begin{figure}[ht]
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.4\textwidth]{figures/exampletree.pdf}
	\caption{Tree topology for seven processes}
  \label{fig:exampletree}
\end{subfigure}
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.8\textwidth]{figures/threephase.pdf}
	\caption{Communication pattern with a tree topology for seven processes ($p_0$ --- $p_6$) and one client ($C$)}
  \label{fig:threephase}
\end{subfigure}
\caption{Tree topology and communication pattern for seven processes.}
\label{fig:tree}
\end{figure}

When using a tree to implement \textsl{disseminate-to-followers} and \textsl{aggregate-at-leader}, the notion of robust configuration needs to be adapted. In fact, in a tree, it is not enough that the leader is non-faulty to make the configuration robust. Instead, the communication graph (in our case, the communication tree), must be robust. We define a \textit{robust graph} as follows.

\begin{definition}
\textbf{Robust Graph:} An edge is said to be \textit{safe} if the corresponding vertices are both correct processes. A graph is robust iff the leader process is correct and, for every pair of correct process $p_i$ and $p_j$, there is a path between $p_i$ and $p_j$ composed exclusively of safe edges\label{def:robust}
\end{definition}


\subsection{Achieving Reliable Dissemination and Fulfillment}

In the following we describe how to implement \textsl{disseminate-to-followers} and \textsl{aggregate-at-leader} on a tree such that Reliable Dissemination and Fulfillment are satisfied. We start by describing the communication primitives used to propagate information on the tree and the cryptographic primitives used to perform aggregation.

\subsubsection{Communicating on the Graph}
Processes use the overlay network to communicate. 
%Each edge in the graph corresponds to a perfect point-to-point channel that is used by neighbor processes to communicate.  
Each directed edge maps to a perfect point-to-point channel that is used at most once, to send and deliver a single value. Perfect point-to-point channels expose a \textsc{send} primitive used to send a message, and a \textsc{deliver} primitive used to receive a message, and exhibit the following properties.

\begin{itemize}
    \item \emph{Validity:} If a process $p_j$ delivers a value $v$ on a channel over an edge $e_{ij}$, $v$ was sent by $p_i$.
    \item \emph{Termination:} If both $p_i$ and $p_j$ are correct, if $p_i$ invokes \textsc{send} then eventually $p_j$ delivers $v$.
\end{itemize}

%When using the overlay to aggregate information, nodes wait for their children to propagate data upstream. Conversely, when the overlay is used to dissiminate information, nodes wait for their parents to propagate downstream. For liveness, the aggregation/dissemination process must proceed even in the occurrence of faults. 
Note that, when using perfect channels, a message is only guaranteed to be eventually delivered if both the sender and the recipient are correct. If the sender is faulty, no message may ever be delivered. To avoid blocking, a process should be able to make progress if a message takes too long to be received.

This behaviour is captured by an abstraction we call \textit{impatient channels}. Impatient channels offer a blocking \textsc{receive} primitive that always returns a value: either the value sent by the sender, or a special value $\bot$ if the sender is faulty or the system is unstable. After the Global Stabilization Time (GST)\cite{partial}, if the sender and the receiver are correct, the receiver always receives the value sent. Impatient channels have the following properties:

\begin{itemize}
    \item \emph{Validity:}  If a process $p_j$ receives a value $v$,  $v$ was sent by a process $p_i$ or $v=\bot$.
    \item \emph{Termination:}  If a correct process $p_j$ invokes \textsc{receive}, it eventually returns some value.
    \item \emph{Conditional Accuracy:} Let $p_i$ and $p_j$ be correct sender and receiver processes, respectively. After GST, $p_j$ always return the value $v$ sent by $p_i$.
\end{itemize}

Algorithm~\ref{algo:impchannels-receive} shows how impatient channels can be implemented on top of perfect channels using the known bound $\Delta$ on the worst-case network latency.

\setlength{\textfloatsep}{0pt}
\begin{algorithm}[t]
\scriptsize
\centering
\caption{Impatient Channels: implementation of \textsc{receive}}
\label{algo:impchannels-receive}
\begin{algorithmic}[1]

\State{let \textit{ic} be an impatient channel built on top of perfect channel \textit{pc}}
\Function{\textit{ic}\textsc{.receive}}{ }
\State{\textsc{timer.start}($\Delta$)}
\When{\textit{pc}.\textsc{deliver} ($v_i$)}
    \State{\Return $v_i$}
\EndWhen
\When{\textsc{timer.timeout}()}
    \State{\Return $\bot$}
\EndWhen
\EndFunction
\end{algorithmic}
\end{algorithm}
\setlength{\textfloatsep}{5pt}

\subsubsection{Cryptographic Collections}

In each phase of the consensus protocol, it is necessary to collect a Byzantine quorum of votes. The collection and validation of these votes can be an impairment for scalability. \thesystem mitigates these costs by using the overlay network to aggregate votes as they are forwarded to the leader. We model the process of aggregation of votes with abstraction called a \textit{cryptographic collection}, which corresponds to a secure multi-set of tuples $(p_i, v_i)$. A process $p_i$ can create a new collection $c$ with a value $v_i$ by calling $c$=\textsc{new}($(p_i, v_i)$). Processes can also merge two collections using a \textsc{combine} primitive,  $c_{12}$ = \textsc{combine}$(c_1, c_2)$, also denoted by $c_{12} = c_1 \oplus c_2$. Finally, a process can check if a collection $c$ includes at least a given threshold of $t$ distinct tuples with the same value $v$, by calling \textsc{has}$(c, v, t)$. Additionally, it is possible to check the total amount of input tuples that were contributed to $c$ by checking its cardinality $\vert c \vert$. Cryptographic collections have the following properties:

\begin{itemize}
    \item \emph{Commutativity:}   $c_1 \oplus c_2 = c_2 \oplus c_1$.
    \item \emph{Associativity:}   $c_1 \oplus (c_2 \oplus c_3)  = (c_1 \oplus c_2) \oplus c_3$.
    \item \emph{Idempotency:} $c_1 \oplus c_1 = c_1$.
    \item \emph{Integrity:} Let $c= c_1 \oplus \ldots c_i \ldots c_n$. If \textsc{has} ($c, v, t$) then at least $t$ distinct processes $p_i$ have executed $c_i$=\textsc{new}($(p_i, v)$).
\end{itemize}

Note that different cryptographic techniques can be used to implement these collections. In \thesystem, we leverage the BLS non-interactive cryptographic aggregation scheme that allows each inner node to aggregate the votes from its children into a single aggregated vote~\cite{bls}. The complexity of verifying an aggregated vote is $\mathcal{O}(1)$, thus the burden imposed on each inner node (including the root) is $\mathcal{O}(c)$, where $c$ is the fanout of the tree.  Note that classical asymmetric signatures require $\mathcal{O}(N)$ verifications at every process and threshold signature schemes require $\mathcal{O}(N)$ at the root and $\mathcal{O}(1)$ at all the other processes~\cite{bls}.

\subsubsection{Disseminate-to-followers}

Algorithm~\ref{algo:disseminate} presents the implementation of \textsl{disseminate-to-followers} on a tree. 
Despite being very simple, we note that the algorithm always terminates, even if some intermediate nodes are faulty. This is guaranteed because impatient channels always return a value after the known bound $\Delta$ on the worst-case network latency, either the \textsl{data} sent by the parent or the special value $\bot$.

\setlength{\textfloatsep}{0pt}
\begin{algorithm}[h!]
\scriptsize
\centering
\caption{\textsl{disseminate-to-followers} on a tree (process $p_i$)}
\label{algo:disseminate}
\begin{algorithmic}[1]
\Procedure{\textsl{Disseminate-to-followers}}{$G$, \textsl{data}}
\State{$\textit{children} \gets $ $G$\textsc{.children}($p_i$)} \Comment{Get edges to children of $p_i$}
\State{$\textit{parent} \gets $ $G$\textsc{.parent}($p_i$)} \Comment{Get parent of $p_i$ (returns $\bot$ for root)}
\If{ $\textit{parent} \neq \bot$}
%\For{\textbf{all} $\textit{e} \in \textit{parent}_i$} %\Comment{Empty for root}
    \State {\textsc{channel.receive}(\textit{parent}, \textsl{data})}
    \Comment{Receive from parent}
%\EndFor

\EndIf
\For{\textbf{all} $\textit{e} \in \textit{children}$} \Comment{Send to children}
    \State {\textsc{channel.send}($e$, $\textit{data}$)}
\EndFor
\State{\textbf{return} $\textsl{data}$}
\EndProcedure
\end{algorithmic}
\end{algorithm}
\setlength{\textfloatsep}{5pt}

\begin{theorem}
Algorithm~\ref{algo:disseminate} guarantees Reliable Dissemination.
\end{theorem}

\begin{proof}
We prove this by contradiction. Assume Reliable Dissemination is not guaranteed.
This implies that at least one correct process did not receive the data sent by the leader. This is only possible if: i) at least one correct process is not connected to the leader either directly or through intermediary processes ii) one of the intermediary processes did not invoke \textsc{channel.send} for at least one correct child process iii) the data got lost in the channel.
A Reliable Dissemination implies a robust configuration which following Definition~\ref{def:robust} ensures that the leader is correct and there is a path of correct processes between the correct leader and any other correct process. Therefore the first case is not possible.
Moreover, correct processes follow the algorithm and, because correct processes can only have correct parents in a robust configuration, the second case is also impossible. Finally, the third case is also impossible due to our assumptions on impatient channels.
%However, that directly leads to a contradiction. Since a robust graph is assumed, from 
%that the leader process must be correct and there must be a path of correct processes between the correct leader and any other correct process. Additionally, we assume perfect communication channels making the loss of data impossible.
Therefore, Algorithm~\ref{algo:disseminate} guarantees  Reliable Dissemination.
\end{proof}

\subsubsection{Aggregate-at-leader}

Algorithm~\ref{algo:aggregate} presents the implementation of \textsl{aggregate-at-leader} on a tree. The algorithm relies on the cryptographic primitives to aggregate the signatures as they are propagated towards the root. Like  \textsl{disseminate-to-followers}, \textsl{aggregate-at-leader} always terminates, even if some intermediate nodes are faulty. This is guaranteed because impatient channels always return a value after the known bound $\Delta$ on the worst-case network latency, either the \textsl{data} sent by the children processes or the special value $\bot$. However, before GST or when running using non-robust configurations, the collection returned at the leader may be empty or include just a subset of the required signatures.

\setlength{\textfloatsep}{0pt}
\begin{algorithm}[h!]
\scriptsize
\centering
\caption{\textsl{aggregate-at-leader} on a tree (process $p_i$}
\label{algo:aggregate}
\begin{algorithmic}[1]
\Procedure{\textsl{aggregate-at-leader}}{$G$, \textsl{input}}
\State{$\textit{children} \gets $ $G$\textsc{.children}} \Comment{Get edges to children of $p_i$}
\State{$\textit{parent} \gets $ $G$\textsc{.parent}($p_i$)}\Comment{Get parent of $p_i$ (returns $\bot$ for root)}
\State{$\textit{collection} \gets \textsl{input}$}
\For{\textbf{all} $\textit{e} \in \textit{children}$} \Comment{Empty for leaf nodes}
    \State {\textsc{channel.receive}($e$, \textit{partial})} \label{algo:aggregate-receive}
    \State {$\textit{collection} \gets \textit{collection} \oplus \textit{partial}$}
\EndFor
\If{ $\textit{parent} \neq \bot$}
%\For{\textbf{all} $\textit{e} \in \textit{parent}_i$} \Comment{Send to  parent, if not the root}
    \State {\textsc{channel.send}(\textit{parent}, $\textit{collection}$)} \label{algo:aggregate-send}
\EndIf
%\EndFor
\State{\textbf{return} $\textit{collection}$}
\EndProcedure
\end{algorithmic}
\end{algorithm}
\setlength{\textfloatsep}{5pt}

\begin{theorem}
Algorithm~\ref{algo:aggregate} guarantees Fulfilment.
\end{theorem}

\begin{proof}
We prove this by contradiction. Assume that the leader process was unable to collect $2f+1$ signatures. 
Following Algorithm~\ref{algo:aggregate}, this means that either: i) an internal node did not receive the signatures from all correct children (line~\ref{algo:aggregate-receive}), ii) an internal node did not aggregate and relay the signatures (line~\ref{algo:aggregate-send}), or iii) the leader is faulty. Since we assume perfect point-to-point channels the first case is not possible. The second case may happen, if either the internal node is not a correct process and omits signatures in the aggregate, if it does not relay any signatures, or if it is waiting indefinitely for all answers of its child processes.
Either option leads to a contradiction. Since we assume a robust graph, all internal nodes between the root and a correct process must be correct and hence follow the protocol. Additionally, due to the impatient channels, eventually each channel will return a value to the internal node making sure that eventually it will receive an answer from all child processes (correct or not) allowing it to relay all collected signatures from all correct child processes. Finally, and again because we assume a robust graph, the leader process in a robust graph cannot be faulty.
Therefore Algorithm~\ref{algo:aggregate} guarantees Fulfilment.
\end{proof}

\subsubsection{Challenges of Using a Tree}

We have shown that it is possible to organize nodes in a tree such that, when running in a robust configuration, the use of the tree offers the same guarantees as the star-based pattern used in HotStuff. There are however two main challenges that need to be addressed, in order to make the use of a tree topology a valid alternative:

\begin{itemize}
\item \textit{Define a reconfiguration strategy:} In HotStuff, the configuration is robust if the leader is non-faulty. Therefore, there are only $f$ non-robust configurations and $2f+1$ robust configurations and deriving a reconfiguration strategy that leads to a robust configuration in an optimal number of reconfiguration steps is trivial. When using a tree, a configuration is only robust if the root and all other internal nodes are non-faulty. The total number of configurations and, unfortunately, the number of non-robust configurations, is extremely large. A reconfiguration strategy that is able to guide the system to a robust configuration quickly is non-trivial.
\item \textit{Mitigate the impact of the increased latency:} The use of a tree allows to distribute the load among the participants. Unfortunately, this comes at the cost of increased latency of the \textsl{disseminate-to-followers} and \textsl{aggregate-at-leader} primitives which, in turn, may negatively affect the throughput of the system. An appropriate strategy to mitigate the effects of the additional latency needs to be developed.
\end{itemize}

In the the next sections, we discuss how we address the two challenges above in the design of \thesystem.

